Neural Approaches to Conversational Information Retrieval

A conversational information retrieval (CIR) system is an information retrieval (IR) system with a conversational interface which allows users to interact with the system to seek information via multi-turn conversations of natural language, in spoken or written form. Recent progress in deep learning has brought tremendous improvements in natural language processing (NLP) and conversational AI, leading to a plethora of commercial conversational services that allow naturally spoken and typed interaction, increasing the need for more human-centric interactions in IR. As a result, we have witnessed a resurgent interest in developing modern CIR systems in both research communities and industry. This book surveys recent advances in CIR, focusing on neural approaches that have been developed in the last few years. This book is based on the authors' tutorial at SIGIR'2020 (Gao et al., 2020b), with IR and NLP communities as the primary target audience. However, audiences with other background, such as machine learning and human-computer interaction, will also find it an accessible introduction to CIR. We hope that this book will prove a valuable resource for students, researchers, and software developers. This manuscript is a working draft. Comments are welcome.

==> archive/chapter_CIR.tex <==
\chapter{Conversational Information Retrieval Systems}

This chapter discusses the core components in conversational information retrieval (CIR) systems, with the main focuses on the new challenges raised from the conversational nature in comparison with classic, keyword-based, IR systems. There are three sections in this chapter. The first section describes the general framework of a CIR system; the remaining two present the two core components in the systems, respectively, (1) conversational query understanding and (2) conversational document ranking.

\section{Overview of CIR}

This section first describes the general framework of a typical CIR system, including its core components, the information and data flow, and the differences with keyword-based IR systems. Then, we present an example of a vanilla set-up of a CIR system. This section serves as a reference for the rest of the chapter. 

We will describe the task setting of the TREC Conversational Assistant Track (CAsT), the past TREC Session Track, the shared challenges of the two and the unique challenges of CAsT:
\begin{enumerate}
    \item \cite{kanoulas2012overview} overviews the Session Track.
    \item \cite{carterette2016evaluating} summarizes the evaluation and findings of the Session Track.
    \item \cite{dalton2019overciew} overviews the CAsT Track.
\end{enumerate}


\section{Conversational Query Understanding}
Conversational query understanding differs from the traditional query understanding task in that the former needs to take into account contextual information in conversation history (i.e., query session).
% is a core component and a new challenge of conversational search. 
This section first presents the definition of the task and its available benchmarks. 
Then we present two categories of solutions. One is based on classic IR query understanding techniques (e.g., session-based query expansion), and the other on natural language generation (e.g., contextual query rewriting).

\subsection{Task Definition and Benchmarks}
We first define the conversational query understanding task from different perspectives, ranging from the overall needs to a set of specific mathematical properties.
We then describe available benchmarks and evaluations for query understanding.

\subsection{Classic Query Understanding Techniques in CIR}
We present the following classic IR techniques and their applications in CIR:
\begin{enumerate}
    \item Query Expansion using previous session queries, which is used by Charlie Clark's CAsT participation [Will cite their TREC paper on this when it is out.]
    \item Query and answer expansion using previous interactions, the top performing team from NTU and Waterloo~\cite{yang2019query}.
\end{enumerate}

The NLP style coreference resolution is another popular choice used to resolve the context dependency in CAsT. We will describe the AllenNLP's solution, which is used by CAsT official:
\begin{enumerate}
    \item \cite{lee2017end} leverage neural networks to resolve the coreference in texts.
\end{enumerate}

% \begin{enumerate}
%     \item Session-based query expansion and term re-weighting, and
%     \item Co-references and omission resolution with NLP techniques.
% \end{enumerate}

\subsection{Neural Generation Techniques for Conversational Query Rewriting}

We present the recent development of natural language generation (NLG) techniques and their applications in conversational query rewriting.

We will start with a quick overview of general NLG techniques:
\begin{enumerate}
    \item Seq2seq learning~\cite{sutskever2014sequence}.
    \item GPT-2 and Transformer~\cite{radford2019language}.
\end{enumerate}

Then we define the query rewriting task and how GPT-2 is used in this task:
\begin{enumerate}
    \item The ATeam submission to TREC CAsT which uses vanilla GPT-2 [Wait for their paper]
\end{enumerate}
and 
\begin{enumerate}
    \item how to adapt GPT-2 to the query rewriting task in few shot and zero shot scenario~\cite{Yu2020Rewriter}.
\end{enumerate}



\section{Conversational Document Ranking}

This section presents the task and techniques for conversational retrieval and ranking. We start with the definition of the task, followed by a review of the retrieval and ranking models developed for ad-hoc retrieval, and finally describe the conversational ranking models.

% \subsection{Task Definition and Benchmarks}
% % This section includes:
% \begin{enumerate}
%     \item First, we define the conversational ranking task and its differences with ranking in ad-hoc retrieval. 
%     \item Then, we discuss the benchmarks and evaluation metrics in conversational ranking.
% \end{enumerate}

\subsection{Preliminaries on Ad-hoc Retrieval and Ranking}
We present the necessary background in ad-hoc retrieval and ranking:
\begin{enumerate}
    \item BM25~\cite{croft2010search}
    \item Feature-based ranking models, mainly focus on the pairwise and listwise learning~\cite{liu2009learning}
    \item Neural-network-based ranking models, including CDSSM~\cite{huang2013learning}, K-NRM~\cite{xiong2017knrm}, and BERT~\cite{nogueira2019passage}.
\end{enumerate}

\subsection{Conversational Ranking Models}
We present the conversational ranking models, focusing the discussion on new challenges compared to the models developed for ad-hoc retrieval, including 
% mainly on what is new compared to ad-hoc retrieval models
\begin{enumerate}
    \item Simple vanilla BERT based reranking, as concatenation all previous queries.
    \item Query Rewriting and then use the rewritten query in ad hoc search~\cite{Yu2020Rewriter}
\end{enumerate}

Then we will discuss the additional ways to train the conversational ranker:
\begin{enumerate}
    \item Multi-task learning with query suggestion and contextual ranking~\cite{ahmad2018multi}
    \item RL or Meta learning to directly optimize the query rewriter for the ranking accuracy~\cite{nogueira2017task} and potentially my next paper.
\end{enumerate}
    








==> archive/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> chapter_cir/01_overview.bak.tex <==
% The conversational queries in TREC CAsT are manually curated by the Track organizers to include those dialog phenomena. 
Table~\ref{tab:cast_q} shows two conversational search topics sampled from TREC CAsT 2019 and 2020.
Each topic consists of a title and a detailed description (Desc) which are used as meta-information for evaluation but should not be used by any automatic search systems to be evaluated, and a sequence of conversational queries. 

Compared to ad hoc search, conversational search is unique in search queries. As shown in Table~\ref{tab:cast_q}, the queries for each topic forms a natural conversation session, demonstrating typical dialog behaviors observed in human conversations. For example, a conversational search session typically starts with a query requesting a general introduction about the topic, followed by queries that ask for more information about the topic being discussed, forming an exploratory information seeking trajectory. Topic shift and return are also observed in Table~\ref{tab:cast_q} (b) where PII is discussed in Turn 4 before asking about GDPR again in Turn 5. 

Ellipsis phenomena are frequently encountered in conversational search. 
For example, the query ``what ones reduce it?'' (Turn 7 in Table~\ref{tab:cast_q} (a)) cannot lead to any meaningful search result without knowing what ``ones'' and ``it'' refer to, respectively.
Thus, the search system has to take into account not only the current query but also its conversational context, which includes previous user queries and system responses in the same search dialog session, to identify the user's search intent to retrieve relevant documents. 

Contextual query understanding and conversational document retrieval are the main research topics to be discussed in this chapter.

%They are manually curated by the TREC Conversational Assistant Track (CAsT) organizers.
%Following the TREC format, each topic consists of a title that covers the general scheme of the conversation, a detailed description of the scheme, which provides meta-information for reference but is not supposed to be used by automatic search systems to be evaluated.  The queries of a topic often starts with a general or coarse information needs, involves to more fine-grained information needs, may shift to slightly different subtopics, and forms a natural conversational trajectory. These queries include various dialog phenomena, such as informality, omissions, implied contexts, co-references.


% \cx{To discuss the statistics of CAsT 2019 and CAsT 2020 in contextual dependency types.}
% Table~\ref{tab:cast_q} shows the contextual dependencies in these multi-turn conversational queries. Many turns do not form self-contained queries alone, for example, for the query ``What makes it so unusual''. A direct application of ad hoc search technique on those turns unlikely yields any meaningful results. 
% It is necessary to recover the underlying search intent of each turn using the contextual information in previous query rounds, previous system responses, and may be derived from general common sense knowledge. How to resolve such contextual dependencies in multi-turn conversational queries is one of the main challenges observed in recent conversational search benchmarks.


==> chapter_cir/02_benchmark.bak.tex <==
\section{Benchmarks}
\label{sec:cir_benchmarks}


This section describes in detail two widely used benchmarks of conversational search, the TREC CAsT  benchmark~\citep{cast2019overview, cast2020overview} and the OR-QuAC dataset~\citep{qu2020orqa}. 
They are representative examples of two benchmark construction approaches, TREC and crowdsourcing, respectively.
TREC CAsT is a standard TREC-style benchmark which is constructed by the IR community to evaluate IR systems, following the \emph{test collection evaluation paradigm}~\citep{voorhees2005trec,cleverdon1966factors}. At the core of this  methodology was the idea that live users could be removed from the evaluation loop, thus simplifying the evaluation and allowing researchers to run in vitro–style experiments in a laboratory with just their retrieval engine, a set of queries, a test collection, and a set of judgments (i.e., a list of relevant documents). 
OR-QuAC is an open-domain question answering (QA) benchmark constructed via \emph{crowdsourcing}. 
It is initially curated using crowdsourcing for QA and then extended for the conversational search task by deriving document-level relevance labels from the answer annotations~\citep{chen2017reading}. 
We end this section by briefly reviewing other benchmarks.

\subsection{TREC CAsT}
The TREC Conversational Assistance Track (CAsT) is the result of an IR community's effort of constructing a reusable, standardized, and TREC-quality benchmark for conversational search. As of December 2021, the track has run for three years (in 2019, 2020 and 2021). 
Similar to other TREC tracks, CAsT is an instantiation of a vision shared by the IR community that conversational search is one of the most important themes for building next-generation IR systems~\citep{swirl2018}.

% Being a TREC Track, CAsT provides a reusable benchmark for the community to explore, develop, and measure progress towards the shared vision.
As the first step towards conversational search, CAsT focuses on the document retrieval task, as discussed in Section~\ref{sec:cir_overview}: to retrieve relevant documents (or passages) from a text corpus for a series of conversational queries.


\paragraph{Corpus.} 
The CAsT corpus is a combination of corpora from MS MARCO~\citep{bajaj2016ms} and TREC CAR~\citep{dietz2017trec}. MS MARCO includes an 8-million-passage corpus collected from Bing's QA system when it is originally released by Microsoft. Later, MS MARCO is augmented by a 3.3-million-document corpus constructed by fetching the full content of the URLs associated with those passages~\citep{craswell2019overview}.
The TREC CAR corpus is constructed for the Complex Answer Retrieval Track and includes around 30 million passages collected from Wikipedia. In CAsT 2019 and CAsT 2020, the passage corpora are used and the task is passage retrieval. In CAsT 2021, the task is document retrieval and the MS MARCO document corpus is used.

%information needs, queries, canonical responses
\paragraph{Information Needs.}
The CAsT organizers semi-manually constructed exploratory information needs (topics) from the combination of previous TREC topics, MS MARCO Conversational Sessions, and their own interests and experiences (e.g., they pick queries by themselves or using reference to derived pseudo  search sessions from Bing search logs)~\citep{dalton2019overciew}. 
% One organizer run an embedding based session mining model that identifies coherent and ``conversational-alike''~\cite{rosset2020leading} search sessions from search log, then he manually constructed pseudo conversational search sessions using information needs he abstracted from various user sessions. Then those pseudo conversational search sessions are used by CAsT organizers as references and inspirations when constructing conversational query rounds. 

\paragraph{Conversational Queries.} 
The queries are curated by the CAsT organizers manually. They start from a topic, write an initial query as the first round, and then grow a conversational trajectory with follow-up queries while interacting commercial Web search engines (Google and Bing) (in CAsT 2019) or a baseline search system (in CAsT 2020).
When curating the conversational trajectories, the organizers follow a shared guideline~\citep{cast2019overview} to mimic users' behavior when using a conversational search engine.
As a result, the conversational queries in CAsT reflect the combination of the CAsT organizers' vision of conversational search engines and the conversation behavior of live users of Web search engines.

\input{tables/cast_manualq}

% human de-contextualized queries
\paragraph{Manual Query Rewrites.} 
The conversational queries include various dialog phenomena including co-reference and omission as shown in Table~\ref{tab:cast_q}. 
% though not explicitly emphasized during curation. 
%Besides being informal and concise, a large amount of queries 
These conversational queries require context information from previous rounds to be understood.
To facilitate assessment and research, CAsT also provides an annotated dataset of \textit{manually de-contextualized} queries. 
Table~\ref{tab:cast_manualq} shows the sequence of manually de-contextualized queries for CAsT 2019 Topic 44, 
where each query is rewritten by the organizers to contain all of the information required to represent the single turn of the underlying information need.
%fully represent the intended information needs. These manual oracle queries are available as auxiliary training data and also used to help accessors judge the document relevance. 


% labels, TREC pooling, top K, and human annotation
\paragraph{Relevance Labels.} 
The labels in CAsT are annotated by TREC accessors using the standard TREC \emph{pooling} method. 
The track participants submitted their system's document retrieval results for the given CAsT queries and corpus. The organizers merged the top-$K$ (10 to 15) ranked documents per submitted run to form the \emph{pool} of query-document pairs. TREC annotators accessed the relevance of the pooled pairs and the annotated labels were released as the official TREC benchmark. This TREC-style pooling method was developed to provide robust evaluation of IR systems and has been the standard in the IR community for the past several decades~\citep{voorhees2005trec}.

\paragraph{Advantages.} 
The TREC approach to building IR benchmarks has several advantages.
The information needs are derived from search sessions of real users.
The conversational query rounds are curated to mimic potential user behaviors in a future conversational search engine by IR experts. 
The queries are curated independently with the relevance accessing process, simulating live search scenarios where the retrieved documents of a query are unknown to a user when she forms the query.
The relevance labels allow robust evaluation of different IR systems
because the TREC-style pooling strategy ensures the reusability of TREC benchmarks.
TREC accessors are also well-known to provide high quality annotations.

\paragraph{Limitations.} 
The TREC setup also has some limitations.
The first is the small quantity of the relevance labels, as a trade-off to high quality. 
For example, TREC CAsT consists of in total 100 conversational search topics annotated, each with about ten query rounds. 
This makes TREC CAsT a few-shot setting as the number of labels is insufficient to reliably train any large-scale deep learning models in a supervised learning manner.
The other limitation is that the queries are curated by the CAsT organizers as a reflection of their visions of conversational search. 
As a result, the dataset presents properties and challenges that the organizers considered as important for future CIR systems, but their predictions could be biased.




\subsection{OR-QuAC}

%Compared to the TREC style CAsT benchmark, the OR-QuAC~\cite{qu2020orqa} benchmark is constructed with \textit{crowd sourced} conversational question-answer pairs and derived document level relevance labels from the short answer labels. It is a common approach to construct question answering dataset~\cite{rajpurkar2016squad, choi2018quac, reddy2019coqa} by recruiting  crowd source workers to write questions and to annotate answers. And to derive documents' relevance labels using whether they contain the correct answer phrase for the question is also widely adopted to formulate the Open Domain Question Answering task~\cite{chen17open}. Following these standard approaches, OR-QuAC was gathered by including questions and derives document labels from QuAC~\citep{choi2018quac}, the conversational QA dataset. It also include the manually de-contextualized question annotations from CANARD~\citep{elgohary2019canard}.

Unlike the TREC CAsT benchmark which is constructed semi-manually by IR experts, OR-QuAC is an open-domain conversational question answering benchmark developed via crowdsourcing, as many other recently developed QA benchmarks~\citep[e.g.,][]{rajpurkar2016squad, choi2018quac, reddy2019coqa}.
OR-QuAC is designed for an open-retrieval setting where an IR system to be evaluated needs to retrieve passages from a collection, given a query and its conversational context~\citep{qu2020orqa}. 
OR-QuAC is an extension of the QuAC benchmark~\citep{choi2018quac}, which offers information-seeking conversations, to an open-retrieval setting by (1) creating a collection of over 11 million passages using the Wikipedia corpus that serves as the knowledge source of answering questions, and (2) generating relevance labels for query-passage pairs based on whether the passage contains the answer span of the query~\citep{chen17open}. 
In addition, OR-QuAC aggregates the CANARD dataset~\citep{elgohary2018dataset} which contains context-independent (de-contextualized) rewrites of QuAC queries.   


\paragraph{Conversational Queries.} 
The QuAC query-answer pairs are collected in a process that involves facilitating information-seeking conversations between two crowd workers, a teacher and a student, who discuss a section from a Wikipedia article about an entity~\citep{choi2018quac}. The student is permitted to see only the section’s title and the first paragraph of the article, while the teacher is additionally provided with full access to the section text.  The conversation starts with the student formulating a free-text question (query) from the limited information they have been given. The teacher is not allowed to answer with free text; instead, they must select a contiguous text span in the section. While this decision limits the way answers are generated, it makes evaluation simpler and more reliable. The conversation continues until (1) twelve questions are answered, (2) one of the workers decides to end the interaction, or (3) more than two unanswerable questions were asked.

%The {queries} in OR-QuAC are written by crowd source workers playing a teacher-student collaboration. For every conversation topic, two workers are recruited, one playing the teacher role, the other playing the student role. The conversational topic is about one section of a Wikipedia page. The teacher has access to the section, while the student only have access to the Wikipedia title (the entity), the section title (often an attribute), and the first paragraph of the page which is the general description/definition of the entity. The student starts by writing a question $q$ to ask information in the hidden section, the teacher provides an answer to the question only by selecting a span in the section, and the two continues the question-answering conversation until twelve turns are reached or the conversation fails/ends~\cite{choi2018quac}. The conversations after quality-control cleaning~\cite{choi2018quac} are kept: the student questions are the conversational queries and the teacher answers are answer span labels.

\paragraph{Manual Query Rewrites.} 
%As a dialog between two crowd source workers, 
The queries in QuAC also include ellipse phenomena which make them ambiguous and underspecified, similar to those in CAsT. 
% ~\cite{elgohary2019canard} latter constructed the CANARD dataset which provides the \textit{de-contextualized manual queries} for QuAC questions.
~\cite{elgohary2019canard} recruit a group of crowd workers to manually rewrite the QuAC queries into \emph{de-contextulized} queries that include all the information necessary to understand the information needs. %The rewriting alters as fewer words as possible. 
The resultant CANARD dataset includes manual de-contextualized queries for all QuAC's dev set and a sample of 4,873 conversation topics (34,956) from QuAC's training set.
Then, the QuAC dev set is used as a test set, as the QuAC test set is hidden, and the annotated training topics is split to train/dev with a 9:1 ratio.

\paragraph{Relevance Labels.} 
%The {retrieval label} of OR-QuAC is another addition to QuAC. 
%\cite{qu2020orqa} uses the same approach introduced by (DrQA)~\cite{chen2017reading} and convert the question-answer benchmark to the open retrieval setting. 
An open-retrieval benchmark needs document-level (or passage-level) relevance labels. These can be derived from the query-answer pairs of QuAC using the method proposed by \cite{chen2017reading}. Given a query-answer pair, a passage is labeled as relevant to the query if the answer span occurs in the passage.
%Instead of providing the evidence document directly to the QA system, the open retrieval setting requires the system to first retrieve the evidence document or passage from the corpus and then construct an answer using the retrieved results. This open retrieval setting is closer to real application scenarios and the retrieval-and-answer task is often referred to ``Open Domain QA''.

\paragraph{Corpus.} 
The passage collection of OR-QuAC is constructed by splitting the Wikipedia documents using a standard passage breaker. A passage that appears in the section used in construction and includes the answer span is labeled as relevant to the corresponding query; the rest passages in the corpus are labeled irrelevant to the query. The train/dev/test split follows that of CANARD.


\paragraph{Advantages.} 
A significant advantage of the OR-QuAC benchmark is its quantity. 
As a dataset curated via crowdsourcing, OR-QuAC includes tens of thousands of crowd-sourced question-answer pairs and manually de-contextualized queries.
This is a very valuable resource to train large models for the designated open retrieval task and also to provide (weak) supervision data to develop models for other related tasks. 
For example, CANARD is often used as an additional (weakly supervised) training dataset for improving systems evaluated on TREC CAsT~\citep{cast2019overview}.

\paragraph{Limitations.} 
The major issue of OR-QuAC is data quality. The questions written by crowd workers are of lower quality than the TREC CAsT queries written by IR experts. This is expected because a crowd worker is unlikely to spend as much time as an IR expert in making interesting and challenging information seeking conversations for evaluating IR systems. 
Another issue is that the interactive information-seeking task designed for collecting conversational QA pairs is artificial and does not reflect the complexity of real-world conversational search scenarios. For example, it has been reported that the dialog trajectories in QuAC often follow a pattern that students start dialogs by asking questions about the beginning of the section before progressing to asking questions about the end~\citep{choi2018quac}. 
The setting also ensures that the answer span is in the same document section based on which the question is generated. 
These artifacts can be easily exploited by IR systems to produce good results only on the OR-QuAC benchmark, which are not generalizable to real-world settings.  
In addition, the automatic relevance labeling process is problematic. The process labels a passage as relevant to a query based on whether it contains the answer of the query. However, the passage that contains the answer span might not be truly relevant if it does not include enough evidence to answer the question. On the other hand, there could be many relevant passages that do not contain the answer span.

%The {challenges} of OR-QuAC are main associated with its crowd-source process and post-constructed retrieval labels. The questions written by crowd-source workers are of a lower quality than those by experts. For example, it is not expected a worker would spend a large amount of time to consider what is a more interesting and challenge conversational trajectory for benchmarking. It is observed that the trajectory often follows a pattern that starts from the beginning of the section and moves to later sentences linearly~\cite{choi2018quac}. The set up of the question curation also guarantees the relevant passages of all queries in a conversation topic resides in the same section of the topic entity's Wikipedia page.  Both patterns lead to certain dataset artifacts and can be exploited by systems with specifically designed features, which may not generalize to real conversational search scenarios. 
%In addition, the construction of the open retrieval labels also leads to a denotation problem: the relevant passage automatically labeled by answer span containment is often not the only relevant passage for the query. At the same time there could also be passages that contain the answer span but not include enough evidence to actually answer the question.

\input{tables/convsearch_datastat}
\input{tables/convdataset_properties}
% \cx{here: 1) to recap the stats and 2) to sum up the good and the bad, perhaps by another table.}

The statistics of the CAsT and OR-QuAC benchmarks are listed in Table~\ref{tab:convsearch_dataset}. Their notable properties are summarized in Table~\ref{tab:convdataset_properties}. Note that we discuss the limitations of these benchmarks not to discourage the use of them, but to raise the awareness of potential misjudging the effectiveness of the search methods being evaluated due to these limitations.
A technique does not work well on CAsT only because there is no sufficient training signals in CAsT.
A technique that uses spurious information (e.g., the description of a CAsT topic, or the design constrain that all relevant passages of a OR-QuAC topic are from the same Wiki page section) could have shown artificially high performance on these benchmarks but it is unlikely to generalize well to real scenarios.
``All benchmarks are wrong, but some are useful''\footnote{\url{https://en.wikipedia.org/wiki/All\_models\_are\_wrong}}. 
It is important to understand the pros and cons of a benchmark before it can be correctly used to evaluate research progress.

\subsection{Other Related Resources}
Besides TREC CAsT and OR-QUAC, there are many other datasets and resources related to conversational search.
The first group of related resources are the OpenQA benchmarks, which consist of single round questions, answer labels, and open retrieval labels. 
These benchmarks include the open-retrieval version of SQuAD~\citep{chen2017reading, lee2019latent}, TriviaQA~\citep{joshi2017triviaqa}, and Natural Questions~\citep{natural-questions}.
The second group of related resources are the ad hoc search benchmarks that include single round queries and relevance documents or passages. 
The most notable one is MS MARCO~\citep{bajaj2016ms}, which is one of the largest search relevance benchmark.
Both OpenQA and search datasets are frequently used as additional (weak) supervision data in conversational search.
Recently, the QReCC dataset~\citep{anantha2020open} is released as yet another conversational search benchmark. It extends CAsT and QuAC with additional dialogs constructed from Natural Questions and additional passages sampled from Common Crawl.





==> chapter_cir/03_preliminary.bak.tex <==

\section{Pre-Trained Language Models}
\label{sec:cir_preliminary}

Before discussing recent progress in conversational search, we first introduce pre-trained language models (PLMs), which have been adopted in nearly all the components of CIR systems, including  conversational search. In fact, many recent advances in CIR are attributed to PLMs. 

Language model pre-training is an active research field. A recent survey is \cite{xu2021pre}.
% We refer interest readers to ~\cite{devlin2018bert, liu2019roberta, raffel2019exploring,xu2021pre} for more information.
In this section we describe BERT~\citep{devlin2018bert}, a classic PLM based on the Transformer architecture~\citep{vaswani:17}, and the pre-training and fine-tuning framework that has been widely used to adapt a PLM to downstream applications.


\subsection{BERT: A Transformer-Based PLM}
A Transformer is a deep learning model that adopts the self-attention mechanism to differentially weight the significance of each part of the input data. 
Transformer models have been proved effective in performing a wide range of natural language and computer vision tasks, and stable and robust in large-scale model training. 
Thus, Transformer becomes the de facto neural architecture for PLMs.
%Here we recap the orignal configuration of Transformer~\cite{vaswani:17} with the updated position embedding formulation in BERT by Delvin et al.~\cite{devlin2018bert}. This vanilla setup is widely used in many language systems, often found the most effective among various latter Transformer variants, too~\cite{narang2021transformer}.

In the rest of the chapter, we use the following equations to denote the text encoding process using a Transformer-based PLM,
%
\begin{align}
    X &\xrightarrow{\text{Transformer}} \mathbf{H}, \text{or} \\
    \mathbf{H} &= f_\text{Transformer}(X),
\end{align}
%
where an input token sequence $X=\{x_1,...,x_i,...,x_n\}$, where $x_i$ is a sub-word (e.g., a BPE token~\citep{sennrich2015neural}), is encoded by a sequence of contextualized dense representation vectors $\mathbf{H}=\{\mathbf{h}_1,...,\mathbf{h}_i,...,\mathbf{h}_n\}$.

Now, we describe the encoding process in detail. As an example, we consider BERT (Bidirectional Encoder Representations from Transformers), one of the most widely used Transformer-based PLMs. 
BERT makes use of the attention mechanism of Transformer to learn contextual relations between words (or sub-words) in a text. In its vanilla form, Transformer includes two separate modules — an encoder that reads the text input and a decoder that produces a prediction for the task. Since BERT is an autoencoding language model, only the encoder module is needed.

BERT performs encoding in two steps: (1) input embedding using an embedding layer, and (2) contextualized encoding using a stack of Transformer layers. 
%This process goes through two components of the networks: an input layer the embeds discrete tokens, and a series of stacked Transformer layers to product contextualized representations.

\paragraph{Embedding Layer.} 

The embedding layer converts the input sequence of discrete tokens to a sequence of continuous embedding vectors. 
As illustrated in Figure~\ref{fig:bert-input}, for a given token, its embedding vector is constructed by summing the corresponding token, segment, and position embeddings.
The Transformer in its vanilla form~\citep{vaswani:17} uses relative position embeddings while BERT uses absolute position embeddings, and DeBERTa, a recent variant to BERT, uses disentangled position embeddings~\citep{he2020deberta}.

\begin{figure}[t] 
\centering 
\includegraphics[width=0.8\linewidth]{fig/bert-input.jpg}
\vspace{-1mm}
\caption{The BERT input embeddings are the sum of the token embeddings, the segmentation embeddings and the position embeddings. Figure credit: \cite{devlin2018bert}.} 
\label{fig:bert-input}
\vspace{0mm}
\end{figure}

%\begin{align*}
%    \bs{x}_i &= \bs{x}'_i + \bs{i}; \bs{x}'_i = f_{\text{word emb}}(x_i);    \bs{i} &=f_{\text{pos emb}}(i).
%\end{align*}
%Here $\bs{x}'_i, \bs{i} \in R^d$ are embedding vectors of the discrete token $x_i$ and the discrete position id $i$, produced by the standard embedding layers $f_{\text{word emb}}$ and $f_{\text{pos emb}}$ which learn a continuous vector for each word and position, correspondingly. The two embedding vectors are summed together to produce the positional-aware token embedding $\bs{x}_i$. The position embedding is the only place where the Transformer accesses and models the sequence order information.

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/transformer-architecture.PNG}
    \caption{
    (Left) Scaled dot-product attention. 
    (Middle) Multi-head attention consists of several attention layers running in parallel. 
    (Right) The Transformer encoder. 
    Figure credit:~\cite{vaswani:17}.}
    \label{fig:Transformer}
\end{figure}

\paragraph{Transformer Layers.}

The embedding vectors are then fed into a stack of Transformer Layers to produce contextualized representations. 
Each Transformer layer has two sub-layers comprising a multi-head attention layer followed by a position-wise feed forward network, as depicted in Figure~\ref{fig:Transformer} (Right).

The attention function used by the Transformer is called \emph{Scaled Dot-Product Attention}, as illustrated in Figure~\ref{fig:Transformer} (Left). The input consists of queries and keys of dimension $d_k$, and values of dimension $d_v$.  In BERT, the embedding vectors of the input (sub-)words serve as the queries, keys and values, and we have $d_k = d_v = d$. To compute the attention functions on each input token, the queries, keys and values are packed together into matrices $\mathbf{Q}$, $\mathbf{K}$, $\mathbf{V}$. The attention matrix is computed as

\begin{equation} \label{eqn:ch3-transformer-attention}
\text{Attention}(\mathbf{Q},\mathbf{K},\mathbf{V}) = \text{softmax} \left( \frac{\mathbf{Q} \mathbf{K}^{\top}}{\sqrt{d_k}} \right) \mathbf{V},
\end{equation}
%
where $\sqrt{d_k}$ is the scaling factor of dot-product (multiplication) attention. 

Instead of performing a single attention function with $d$-dimensional keys, values and queries, \cite{vaswani:17} propose to perform \emph{Multi-Head Attention}, as illustrated in Figure~\ref{fig:Transformer} (Middle). 
It first linearly projects the queries, keys and values multiple times with different, learned linear projections to $d$ dimensions. Then, on each of these projected versions of queries, keys and values, the scaled dot-product attention function is performed in parallel, yielding $d$-dimensional output values. These are concatenated and once again projected, resulting in the final values.

\begin{align} \label{eqn:chp3-transformer-multi-heand-attention}
\text{MultiHead}(\mathbf{Q},\mathbf{K},\mathbf{V}) &= \text{Concat} \left(\text{head}_1,...,\text{head}_H \right) \mathbf{W}^O, 
\\
\text{head}_i &= \text{Attention}(\mathbf{Q}\mathbf{W}_i^Q, \mathbf{K}\mathbf{W}_i^K,  \mathbf{V}\mathbf{W}_i^V),
\end{align}
%
where $\mathbf{W}$’s are trainable parameter matrices.

%Each Transformer layer takes the output of its previous layer $\mathbf{H}_{l-1}$ and uses an attention mechanism to produce $\mathbf{H}_{l}$:

%\begin{align}
%    \bs{H}^l &= \bs{W}^{F} \cdot \text{softmax}(\frac{\bs{Q} \cdot \bs{K}^T}{\sqrt{d}}) \cdot \bs{V}^T,   \\
%    \bs{Q}^T;& \bs{K}^T; \bs{V}^T=\bs{W}^q \cdot \bs{H}^{l-1}; \bs{W}^k \cdot \bs{H}^{l-1}; \bs{W}^v \cdot \bs{H}^{l-1}, \\
%    \bs{H}^0_i &= \bs{x}'_i. 
%\end{align}
%It includes three projections ($\bs{W}^q, \bs{W}^k, \bs{W}^v$) on the input $\bs{H}^{l-1}$ to produce three matrices: Query ($\bs{Q}$), Key ($\bs{K}$), and Value ($\bs{V}$). Each row in these matrices corresponds to a position in the text sequence and forms the attention mechanism per-token-wise as:
%\begin{align}
%    \bs{h}_i^l &= \bs{W}^F \sum_j \text{softmax}_j(\frac{\bs{q}_i^T \cdot \bs{k}_j}{\sqrt{d}}) \cdot \bs{v}_j.\label{eqn:att}
%\end{align}
%It first calculates the attention of token $i$ to all other tokens $j$ in the sequence and then combines the token values $\bs{v}_j$ into a new representation $\bs{h}_i^l$, using the normalized attention weights. The normalization (with square root of the vector dimension $\sqrt{d}$) help improve numeric stability. The aggregated new representations also pass through another project layer $\bs{W}^F$ to obtain the final output representation $\bs{H}_l$ of this Transformer layer. Often the query, key, and value vectors in Eqn.~\ref{eqn:att} are split into groups when calculating the softmax, i.e., to make the attention ``multi-head'', which increases the capacity of the attention mechanism. 

%Note that in Eqn~\ref{eqn:att}, each token can attend to all other positions, both on its left and right in the sequence. Such ``bi-directional'' Transformer encoders are more effective in representing natural language, in comparison to ``uni-directional'' networks where tokens are restricted to only attend to tokens either on its left or right. The latter is more suitable for language generation tasks.

%Figure~\ref{fig:transformer-architecture} illustrate the attention mechanism, the stacked multi-head attention, and the full Transformer encoder network. Standard techniques that help neural network training, e.g., as residual connections~\cite{he2016deep} and layer normalization~\cite{ba2016layer}, are also used throughout the network. 

%In the rest of this book, we will use the following two notations to refer to the process of using a Transformer network to convert text sequence $X$ to contextualized representation $\bs{H}$
%\begin{align}
%    X &\xrightarrow{\text{Transformer}} \bs{H}, \text{or} \\
%    \bs{H} &= f_\text{Transformer}(X),
%\end{align}
%where the detailed setup of the Transformer network, e.g., number of layers, architecture variants, is either specified in context or can be interchangeable.



\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{fig/plm-finetune.jpg}
    \caption{The pre-training and fine-tuning framework.}
    \label{fig:plm-frame}
\end{figure}


\subsection{Pre-Training and Fine-Tuning Framework}
Training a deep Transformer model from scratch requires a large amount of labels that is only available in a few applications, such as machine translation where millions of parallel sentences can be used for training~\citep{vaswani:17}. A more efficient method is to first \emph{pre-train} a Transformer-based language model on raw text corpora via self-supervised learning ~\citep{devlin2018bert, liu2019roberta}, and then \emph{fine-tune} the pre-trained language model to downstream tasks with limited amounts of task-specific labels. 

Figure~\ref{fig:plm-frame} illustrates the 
\emph{pre-training and fine-tuning} framework. 
%One can view it as a form of unsupervisedly/weakly-supervised learning: first training on a large amount of unsupervised signals and then with supervised labels. 
This is an instance of transfer learning, where the knowledge learned by the PLM for a language modeling task (e.g., masked language modeling) is transferred to perform a different downstream task.
In this section we review the masked language modeling task used for BERT pre-training~\citep{devlin2018bert}, and then discuss several common setups to fine-tune PLMs to downstream tasks.

\paragraph{Pre-training with Masked Language Modeling.}
The Masked Language Modeling (MLM) task can be illustrated as

\begin{align*}
    \texttt{[CLS]}, x_1, \dots, \texttt{[MASK]}_i, \dots, x_n \xrightarrow{\text{Transformer}} \mathbf{H} \xrightarrow{\text{MLM head}} p_{\text{MLM}} (x_i | \mathbf{h}_i).
\end{align*}
%
Before feeding word sequences $X=\{x_1,...,x_n\}$ into BERT, 15\% of the words in each input sequence are replaced with a \texttt{[MASK]} token. The model then attempts to predict the original value of each masked word $x_i$, based on its contextualized representation $\mathbf{h}_i$, which encodes context provided by the other, non-masked, words in the sequence. 
\texttt{[CLS]} is a special token, added at the beginning of an input sequence, to produce the representation of the entire sequence, which is useful for many downstream tasks.
Technically, the prediction of the output words requires adding, on top of the encoder output, an MLM head, which is a classification layer that multiplies the output vectors $\mathbf{x}_i$ by the embedding matrix, transforming them into the vocabulary dimension $|\mathcal{V}|$, and calculates the probability of each word in the vocabulary with softmax as

\begin{align*}
P_r (x | \mathbf{h}_i) = \frac{\exp(\mathbf{x}^\top \mathbf{h}_i)}{\sum_{x_t \in \mathcal{V}} \exp(\mathbf{x}_t^\top \mathbf{h}_i)}.
%\quad
%\mathcal{L}_\text{MLM} = \mathbb{E} \left( - \sum_{i\in %\mathcal{M}} \log  p_{\text{MLM}} \left( x_i \big| \bs{h}_i %\right) \right).
\end{align*}
%

%Language modeling is a classic  language task. It can be abstracted as to predict some words in a natural language sequence using the rest words as inputs. The traditional language model task is often termed as ``auto-regressive'', as the language model is to predict the next token using all previous tokens. It is intuitive as it follows the natural language flow but may not be as suitable to train the bi-directional encoder. The masked language modeling task~\citep{devlin2018bert}, on the other hand, is to randomly mask a fraction of tokens in the input sequence (often 15\% empirically) and to predict them using the rest tokens from both directions. It is more suitable to train the bi-directional Transformer encoders.

%Specifically, the masked language modeling task (MLM)~\citep{devlin2018bert} is to take an input text sequence $X=[x_1,\dots,x_i,\dots,x_n]$, with random tokens at positions $i\in  \mathcal{M}$ replaced by mask symbols ``$\texttt{\_}$'', and to predict the masked out tokens at those positions:

% where the Transformer generates contextualized representations $\bs{H} = \{\bs{h}_i\}_{i=1}^n$. 

%The MLM head is a language modeling layer applied on $\bs{h}_i$, the Transformer's contextualized representations on the masked positions, to predict the original tokens from the vocabulary $V$:

\begin{figure}
    \centering
    \includegraphics[width=0.70\textwidth]{fig/BERT-MLM.jpg}
    \caption{Pre-training BERT with Masked Language Modeling~\citep{devlin2018bert}.}
    \label{fig:BERT}
\end{figure}

Figure~\ref{fig:BERT} shows an example of pre-training BERT using MLM. Since no manual label is required, BERT can be trained on large amounts of raw text corpora. 
%The language modeling task uses natural language texts as their training data, thus benefits from near infinite pretraining signals.
For example, the BERT base model, a 12-layer Transformer with 110 million parameters, is pre-trained on the Wikipedia and Google Book Corpora which amount to 16 GB words~\citep{devlin2018bert}. 
Recent results show that training a larger PLM on a larger dataset significantly improve model's performance, especially in few-shot or zero-shot settings where there is few or zero task labels for fine-tuning the model to a downstream task~\citep{liu2019roberta, raffel2019exploring,brown2020language,roberts2020much,schick2020s}.

While the root reason why PLMs are so effective remains an open research topic, a recent study shows that BERT does capture linguistic information, representing the steps of the traditional NLP pipeline (e.g., POS tagging, parsing, NER, semantic roles, then coreference) in an interpretable and localizable way~\citep{tenney2019bert}.

%Though it is still being investigated what information is learned in pretrained language models, empirically they  are widely observed effective in capturing certain language syntactic and semantic, for example, those modeled in classic NLP pipelines~\cite{tenney2019bert}. 
%Their few-shot or even zero-shot prediction power from these pretrained models with prompt-based learning also indicates much useful information is captured in their pretrained weights~\citep{brown2020language, roberts2020much,  schick2020s}. These information captured during the pretraining process provides significantly boost of the neural network's effectiveness when fine-tuned in the downstream applications.


\paragraph{Fine-Tuning for Downstream Tasks.}

A PLM can be adapted to downstream tasks by continually fine-tuning the parameters of the PLM and an added task-specific head using task labels, e.g., relevance labels in document search. 
Depending on the formulation of the target downstream task, we use different types of task-specific heads, and process training data accordingly.
% and to add task specific layers on the output representations of the neural networks.
Figure~\ref{fig:plm_usage} presents three commonly used formulations of downstream tasks for fine-tuning PLMs.

\begin{figure}
         \includegraphics[width=1.0\textwidth]{fig/PLM-Use.jpg}
            \caption{Three formulations of downstream tasks: single prediction (Left), pair prediction (Middle) and dual-encoding matching (Right).}
     \label{fig:plm_usage}
\end{figure}



The first formulation is \textit{Single Prediction}, as illustrated in Figure~\ref{fig:plm_usage} (Left). It is often used to predict a label for a single text sequence. Take the text classification task as an example. The probability that  text $X$ is labeled as class $y$ (i.e., the positive or negative sentiment) is predicted by a logistic regression with softmax: 
%It feeds the text sequence $X$ to the Transformer and apply a prediction head on its output, e.g., using a linear layer upon the last layer's [CLS] representation:
\begin{align}
    P_r(y|X) = \text{softmax}(\mathbf{W} \cdot \mathbf{x}), \label{eq:single_predict}
\end{align}
where $\mathbf{x}$ is the contextual representation vector of $X$ (i.e., the contextual vector of the \texttt{[CLS]} token), and $\mathbf{W}$ is the task-specific parameter matrix.
Note that we can make prediction using the contextual vectors of other token, rather than \texttt{[CLS]}, in the input. For example, we might want to predict the POS tag of a word or a text span in extractive OA tasks.

The second formulation is \textit{Pair Prediction}, as illustrated in Figure~\ref{fig:plm_usage} (Middle). It is used to predict a label for a pair (or a set) of text sequences. An example is to predict the relevance label of a query-document pair. This can be achieved by feeding the concatenation of query string $X_1$, a \texttt{[SEP]} token, and document string $X_2$ to the model, and the relevance label $y$ is predicted using a logistic regression layer with softmax:
%set of sequences, e.g., query and document, as input to the pretrained Transformer, and uses a prediction layer on the output [CLS] representation:
\begin{align}
    P_r(y|X_1, X_2) = \text{softmax}(\mathbf{W} \cdot \mathbf{x}),
    \label{eq:pair_predict}
\end{align}
where $\mathbf{x}$ is the contextual representation vector of the concatenated input sequence (i.e., the contextual vector of the \texttt{[CLS]} token), and $\mathbf{W}$ is the task-specific parameter matrix.
%[SEP],another special token, marks the boundary between sequences. In search ranking, query is $X_1$, document is $X_2$ and $n=2$. Often one Linear layer on top of [CLS] is sufficient; most of the model capacity is in the Transformer networks. 
In neural IR, this pair prediction task is sometimes denoted as BERT$_\text{CAT}$ or Transformer$_\text{CAT}$.

The third formulation is \textit{Dual-Encoding Matching}, as illustrated in Figure~\ref{fig:plm_usage} (Right). This is often used in text similarity or matching tasks. For example, in document search, we might want to compute the relevance score Rel(.) between query $X_1$ and each candidate document $X_2$ as
\begin{align}
    \text{Rel}(X_1, X_2) = \text{sim}(\mathbf{x}_1, \mathbf{x}_2;\theta),
    \label{eq:dual_encoding}
\end{align}
where $\mathbf{x}_1$ and $\mathbf{x}_2$ are the contextual representation vectors of $X_1$ and $X_2$, generated by the two encoders (dual-encoding), respectively, and sim(.) is a similarity function which can be implemented using cosine similarity or a model parameterized by $\theta$.
%one first encodes the query and documents and then retrieves the nearest neighbor documents of the given query in the embedding space~\cite{lee2019latent, karpukhin2020dense, xiong2020approximate}. 
Compared to the pair prediction formulation, dual-encoding is more often used for document retrieval where runtime efficiency is important. Dual-encoding allows documents and queries to be encoded separately so that we can \emph{pre-encode} all documents and then the IR system only needs to encode an input query on the fly for retrieval. Dual-encoding is widely used for dense retrieval~\citep{huang2013learning, lee2019latent, karpukhin2020dense, xiong2020approximate}, which will be discussed in the next sections. 
This formulation is also referred to as the representation-based model, dual-encoder, siamese-encoder, weak interaction model, deep structured similarity model etc.

%The efficiency constraints make it necessary to encode sequences (e.g., queries and documents) individually, and then matches them purely by their embedding similarities:
%\begin{align}
%    f(X_1, X_2) &= \text{sim}(\text{Transformer}_\text{REP}(X_1), \text{Transformer}_\text{REP}(X_2)).
%\end{align}
%The choice of the similarity function (sim) is restricted to those supported by efficient nearest neighbor search toolkits, such as cosine similarity, dot product, and L2 distance~\cite{FAISS}. 
%There are many terminologies used to refer to this setup, for example, ``representation-based model'', Dual-Encoder,  Siamese-Encoder, weak interaction model, etc. The encoders ($\text{Transformer}_\text{REP}$) used on the two sequences may share the same parameter weights or be completely different. No prediction head is used. All model capacity is in the encoders.

The PLM fune-training follows the standard supervised learning procedure, where the parameters of the PLM and its added task-specific head are optimized w.r.t. the task loss, e.g., cross entropy for prediction, rank loss in relevance ranking, and NCE loss in dense retrieval. 









==> chapter_cir/04_architecture.bak.tex <==
\section{System Architecture}
\label{sec:convsearch_arch}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/document-search-arch.jpg}
    \caption{ A general architecture of conversational document search systems. \label{fig:document-search-arch}}
\end{figure}

%This section presents a system architecture commonly used in current conversational search systems. We first present an overview of a typical system and then describe the task and challenge of its each individual component. 
%The notations used in this section and the rest of the chapter are listed in Table~\ref{tab:convsearch_notation} for reference.

A typical architecture of conversational search systems is illustrated in Figure~\ref{fig:document-search-arch}. It consists of a subset of the components of Figure~\ref{fig:cir-system-arch}.
Following the task setting described in Section~\ref{sec:cir_overview}, conversational search is performed as follows.
A user issues a series of conversational queries $\{Q_1,...,Q_N\}$ for a topic $\mathcal{T}$, where each query $Q$ is part of the conversational trajectory and its answer depends on not only $Q$ but its dialog history $\mathcal{H}$ which includes all its previous queries and their system responses.
The system returns for each query $Q$ a list of documents $\{D_1,...,D_M\}$, ranked by their relevance scores with respect to $Q$.
The search is conducted using three components: contextual query understanding, document retrieval, and document ranking. 
The result generation module will be discussed in Chapters 5 and 6. 

%\textbf{Overall Architecture.} 
%A common pipeline of conversational search system are illustrated in Figure~\ref{fig:convsearch_arch}. As discussed in previous sections, in conversational search, a user provides a series of conversational queries $\{q_1,...q_i...,q_n\}$ for a topic $\mathcal{T}$, where each $q_i$ is part of a conversational trajectory and may depend on contexts in previous turns, and the system is to retrieve and rank a list of document $\{d^i_1,...d^i_j...,d^i_m\}$ for each turn $q_i$. Many current conversational search systems can be viewed as processing a such search request via four components: \textit{Contextualized Query Understanding}, \textit{Document Understanding}, \textit{First Stage Document Retrieval}, and \textit{Document Ranking}. In Figure~\ref{fig:convsearch_arch}, we illustrate the system architecture of a viable conversational search system with these four components, which we describe next.

\paragraph{Contextual Query Understanding.} 
Since ellipsis phenomena are frequently encountered in conversational search, understanding a conversational query $Q$ relies on its context.  
Contextual query understanding conceptually acts as a query rewriter, which uses contextual information of dialog history $\mathcal{H}$ to rewrite $Q \in \mathcal{T}$ to a de-contextualized query $\hat{Q}$ for document retrieval. 
The rewriter can be implemented as a separate module using query expansion methods or neural rewriting models (Section~\ref{sec:cqu}), or as part of the conversational dense retrieval module (Section~\ref{sec:conv_dense_retrieval}). 

%Given a user input natural language query $q$, the query understanding component is to convert the query into a computer understandable query, often in a vector format $\bf{q}$, which can either be a one-hot vector in the sparse word space, or a dense embedding vector. One main challenge of query understanding in conversational search is to effectively represent user's information needs in the concise and contextually dependent query. This is a unique challenge in conversational search and has been one of the main research focus in conversational search.

%\textbf{Document Understanding.} Similar to the query side, the search system need to convert the text documents into a vector representation space, discrete or continuous. Different from query representation, document representation is often conducted offline thus has less efficiency constraints. Also, to effectively represent the information in the document encounters different challenges in representing the query. Different techniques are required on the two sides.

%Currently, many conversational search systems treat the document representation the same as in an ad hoc search system. It is intuitive as the information stored in a document is the same regarding to different search formats.

\paragraph{Document Retrieval.} 
Identifying a short list of relevant documents of query $Q$ (or its de-contextualized form $\hat{Q}$) from a large document collection $\mathcal{D}$ is computationally expensive. For efficiency, a coarse-to-fine search strategy is widely adopted where the overall search process is divided into two phases, document \emph{retrieval} and \emph{ranking}, either of which may consist of multiple steps to perform coarse-to-fine document retrieval or (re-)ranking, respectively. 

Conceptually, document retrieval needs to examine each $D \in \mathcal{D}$ its relevance to $Q$. Since a brute-force method is prohibitively expensive,
it is necessary to construct an index of $\mathcal{D}$ for efficient retrieval. 
For example, sparse retrieval methods (Section 3.6) often use the (weighted) inverted index to help find the top-$K$ relevant documents efficiently, as that in ad hoc search~\citep{croft2010search}.
Dense retrieval methods (Section 3.7), on the other hand, have to resort to efficient similarity search methods \citep{aumuller2017ann,FAISS,li2020improving} to find relevant documents in a continuous vector representation space.   
% The actual search process in conversational search follows the standard cascade information retrieval pipeline, which includes multiple steps of retrieval and reranking to zoom in a smaller and smaller set of candidate documents till the final ranking results are produced.
%The first step is significantly different from the latter ones as the system needs to find a set of relevant candidate documents for the query in the entire corpus. Given the size of most search corpora, it is infeasible to enumerate all the documents one by one and calculate their relevance score for a given query. Often it is necessary to construct an index of the corpus and efficiently match the query with the index, for example, in the vector representation space, to retrieve top K (often in the thousands) documents~\cite{croft2010search}. This step is referred as ``retrieval'' or ``first stage retrieval'' in the information retrieval and natural language processing community.
%The first stage retrieval in conversational search is usually conducted similarly with that in ad hoc search, as the retrieval function itself is bounded to be simple. The main capacity is in the query representation and document representation parts.

\paragraph{Document Ranking.} 
% After first stage retrieval, the search system can conduct one or multiple steps of reranking, to rank the top K candidate documents for the query.
Given top-$K$ candidate documents retrieved from $\mathcal{D}$, where $K << |\mathcal{D}|$, we can afford to use sophisticated ranking models, such as Transformer-based PLMs, to (re-)rank these documents to return a short list of the most relevant documents to the user.   
%to rerank are provided by first stage retrieval or top K from previous stage reranking when multiple reranking stages are used. As a result, it is more feasible to use more sophisticated ranking models to score each pair of query and candidate document pair, with access to more information and bigger model capacity.

The rest of this chapter describes the models and methods recently developed for the aforementioned three components. %that instantiate these four components based sparse representations (Sec.~\ref{sec:convsearch_bow}) and dense representations (Sec.~\ref{sec:ConvDR}).






==> chapter_cir/05_sparse.tex <==
\section{Sparse Conversational Search Approaches}
\label{sec:convsearch_bow}
In this section, we discuss recent techniques developed for conversational search that are based on sparse term-based text representations. 
Those techniques reside in the standard bag-of-words style information retrieval and are a natural progress of classic information retrieval techniques to conversational search scenarios.

Among the four components categorized in the last section, the first stage retrieval, reranking, and document representation components in sparse token-based conversational search systems often share the same solutions with ad-hoc systems. We  first recap those preliminaries and then discuss various recent techniques are developed in contextual query understanding, 


\subsection{Preliminaries on Sparse Retrieval and Reranking}

Many recent conversational search systems reuse the document understanding, retrieval, and ranking solutions from classical sparse retrieval systems in ad hoc search.
They often first leverage some contextual query understanding techniques to formulate an ad hoc query $q'$, to include all required contextual information, and then a standard ad hoc search system with the reformulated query $q'$. 
This part of this section provide a general recap of the current standard solutions in ad hoc search systems, including first stage retrieval, BERT based reranking, and document expansion. 
% We refer readers to materials dedicated to these ad hoc search techniques for more details.

\textbf{Sparse First Stage Retrieval.} Given a query $q$, the first stage retrieval is to efficiently find a set of relevant documents $D^q$ from the entire corpus $C$. In classic ad hoc systems, this is conducted by matching the bag-of-words (BOW) representation of query and documents using a simple retrieval function:
\begin{align}
    \mathbf{q} &= \{(t, w) | \forall t \in q\} \\
    \mathbf{d} &= \{(t, w) | \forall t \in d\}.
\end{align}
The query and documents are represented as sparse vectors in the high-dimensional space, where each dimension corresponds to a term in the vocabulary, and the term weight $w$ is none-zero only if the term appears in the text. The term weight can be binary, term frequency counts, or learned~\cite{croft2010search}.

Then the retrieval function is to match two sparse vectors efficiently. A popular choice is Okapi BM25:
\begin{align}
    \text{BM25}(q, d) &= \sum_{t\in q} \text{TF}(t, q)\text{IDF}(t, C) \cdot \frac{\text{TF}(t, d)\cdot(k_1 + 1)}{\text{TF}(t, d) + k_1\cdot(1-b+b\cdot\frac{|d|}{\text{avg dl}})}. \label{eq:bm25} \\
    D_\text{BM25}^q &= \text{Top}_k \text{BM25}(q, d). 
\end{align}
The top k highest scored documents with BM25 $D_\text{BM25}^q$ are the output of the first stage retrieval. They can be directly served to the user or passed through more fine-grained ranking models latter. 

 As shown in Eq.~\ref{eq:bm25}, there are three sets of sufficient statistics in the BM25 model:
\begin{enumerate}
    \item Term Frequency: the frequency of a term appearing in the query $\text{TF}(t, q)$ and the document $\text{TF}(t, d)$. The higher the TF, the more important the term is.
    \item Invert Document Frequency: the reverse frequency of a term in the corpus $\text{IDF}(t, C)$. The higher IDF, the rarer a term is and it is considered more informative. 
    \item The document length: the document length $|d|$ and the average document length $\text{avg dl}$ are used to normalize the TF-IDF based score.
\end{enumerate}
The BM25 model was developed by Robertson et al. in the 1970s and 1980s and has been one of the standard sparse retrieval model since then. A more detailed discussion of it can be found in the reprint of their paper~\cite{robertson2009probabilistic}. 

The formulation also introduces a term independent assumption that the relevance score between a q-d pair is a weighted combination of each individual query term's match with the document. This enables efficient retrieval using data structures such as inverted index. There are also various other bag-of-words based retrieval developed in ad hoc retrieval, most of them falls into the same framework and uses the same set of sufficient statistics. 
More details of sparse retrieval and indexing can be found in search engine textbooks~\citep{croft2010search}.


\textbf{BERT-based Ranker.} The reranking task is to further sort the top retrieved documents $D$ from the first stage retrieval, or an earlier reranking stage if multiple reranking steps are employed, that more relevant documents are ranked higher than others. As the candidate documents to rerank are provided and also at a much smaller amount (hundreds or thousands), the ranking step can use more sophisticated models since the efficiency constraints is not as strict.

A common approach for ranking is ``Learning to Rank'' (LeToR)~\cite{liu2009learning}, i.e., to learn a ranking function $f()$ using relevance labels. 
The ranking models can be feature-based statistical machine learning models, such as SVM and Tree models, or later, deep learning models. The latter is coined as ``neural information retrieval'' (Neu-IR)~\cite{mitra2018introduction}. 
As in many other fields, pretrained transformer-based solutions are becoming the new standard in ranking~\cite{lin2020pretrained}. Here we discuss one of the most popular setups of BERT-based rankers and refer to two recent surveys for other Neu-IR solutions~\cite{mitra2018introduction, lin2020pretrained}.

% Soon after BERT is released, 
Nogueira and Cho first provided a simple adaptation of BERT in reranking and demonstrated the advantage of BERT with a big leap on ranking accuracy on MS MARCO~\cite{nogueira2019passage}. The formulation follows the \textit{concatenation and prediction} setup as discussed in Section~\ref{sec:cir_preliminary}:
\begin{align}
    \mathbf{H} &= \text{BERT}_\text{CAT}(\text{[CLS]} \circ q \circ \text{[SEP]} \circ d) \\
    f(q, d) &= \text{Linear}(\mathbf{h}_0).
\end{align}
% It applies BERT on the concatenation ($\circ$) of query and document sequence to obtain a contextualized representation of the pair. Then a simple linear layer is used on top of BERT's [CLS] token representation ($h_0$, the first position of $\mathbf{H}$) to produce the ranking score, exactly the same as how BERT is used on many other NLP tasks~\cite{devlin2018bert}.
The training of the BERT-based ranker simply treats ranking as a binary classification task and fine-tuned the BERT model with binary relevance labels~\cite{nogueira2019passage}, which is the pointwise approach in Learning to Rank~\cite{liu2009learning}.
% However, with BERT the simple classification loss works well.

The BM25 first stage retrieval and then BERT-based reranker is the go-to solution in many ad hoc retrieval systems. Researchers and practitioners in conversational search also leverage this cascade pipeline as the backbone of their search process after formulating an ad hoc de-contextualized query with contextual query understanding.













\textbf{Enriching document representation.} An intrinsic challenge in bag-of-words based sparse retrieval is \textit{vocabulary mismatch}, where their is little overlap between query and relevant documents. One way to mitigate this problem is to use expansion techniques, that enrich the query or document with extra words thus increase the match between them. As many recent conversational search systems share the same document representation with ad hoc search systems, the document expansion techniques developed for ad hoc search can be employed to improve conversational search as well.


In web search engines, the document expansion starts with two valuable sources. The first is anchor texts, the texts associated with hyperlinks pointing to the document, which describes the information in the document from a ``third party'' view.
The second one is click queries, the queries that lead to clicks to the document. The click queries are extremely powerful when available; they reflect user's preference on the document while also easier to match with the current query as they are from the same distribution~\cite{yin2019neural, zamani2018neural}. 

On public benchmarks where search logs are not available, one can approximate the user click queries using language generation. The Doc2Query~\cite{nogueira2019document} method first trains a natural language generation (NLG) model, for example, T5~\cite{raffel2019exploring} using relevant document-query pairs, then uses the NLG model to generate queries for each document for expansion.

An advantage of document expansion techniques is that they are conducted offline thus the efficiency constraint is different from components that have to conducted in online time, for example, reranking or query expansion. As a result, ``heavier'' models can be used. 
On the other hand, document understanding is a challenging topic with various new techniques being developed. Conversational search systems can benefit from those development in ad hoc search and in general language techniques.











\subsection{Conversational Query Expansion Methods}
Equipped with the state-of-the-art solutions in classic sparse ad hoc search systems, in the rest of this section, we introduce recently developed approaches in contextual query understanding in conversational search. In general these approaches aim to convert user's conversational queries into a fully-grown ad hoc query that includes all necessary information for an ad hoc system to find the right documents.
Based on whether the reformed ad hoc target is a bag-of-words query representation or a new natural language query, these techniques can be categorized as either \textit{conversational query expansion}, which we discuss next, or \textit{conversational query rewriting}, which is the focus of the last part in this section.

Given a conversational query $q_i$, the i-th round of the topic $\mathcal{T}$, the sparse query representation task is to find a new query $\hat{q}_i$, either as a bag-of-word vector or as a de-contextualized query, that is an informative standalone query to represent the user's information needs at turn $i$.
Due to the context dependency of conversational queries, it is often necessary to leverage contexts from previous rounds, including the queries $q_{1:i-1}$ and also the system responses $d^{1:i-1}$. 

A popular approach, \textit{Conversational Query Expansion}, or also referred to as Conversational Query Resolution (CQR), is to enrich the user query with terms from previous context that covers the necessary conversational context~\citep{yang2019query, voskarides2020query}. 
Before introducing two approaches for conversational query expansion, we first formally define this task as:

\textbf{Task Definition.} Let $t_k^i$ be the k-th term in query $q_i$, $q_i=\{t_1^i,...t_k^i...,t_K^i\}$, or system response $d_i$ if included, the conversational query expansion task can be view as a binary classification task that select terms from $q_{1:i-i}$ that better conveys user's information needs at turn $i$ when added to $q_i$. From the empirical view, it is to find the best set of terms $S_i$ that:
\begin{align}
    S^*_i &= \text{argmax}_{S_i} \text{Accuracy}(q_i \cup S_i), \label{eq:resotarget}\\
    S_i &= \{t_k^j | t_k^j \in q^j; 1\leq j < i; g(t_k^j)=1\}. \label{eq:expterm_classification}
\end{align}
We use Accuracy($q_i \cup S_i$) to denote the performance of the ad hoc search system when the terms in $S_i$ is added to $q_i$, i.e., to its bag-of-words vector and $g()$ is the target binary classifier to select terms from previous queries and/or turns.

% rather than in ad hoc search where they are often from feedback documents.
Similar to query expansion in ad hoc search~\cite{croft2010search}, it is difficult and often impossible to directly optimize Eqn.~\ref{eq:resotarget}. The ranking system is in general not differentiable. Many approaches are developed to approximate this ideal optimization problem with either unsupervised rules or supervised models with intermediate term level labels. Next we present one representative approach in each category.


\textbf{Unsupervised Historical Query Expansion.}
Lin and Yang et al.~\cite{lin2020multi} developed an interesting heuristic based approach, Historical Query Expansion (HQE), that leverages a base retrieval model as the tool to determine when and which terms to expand the query. A very simple method, it works well empirically and was one of the top performing systems in TREC CAsT 2019~\cite{yang2019query}. 

The HQE method is built upon the following common properties of TREC CAsT conversational search topics observed by the authors:
\begin{enumerate}
    \item Main-Sub Topic Hierarchy: The queries of a conversational session often center around a main topic. Each query turn may shift to a new subtopic or dive deeper in one subtopic.
    \item Ambiguity Categories: The ambiguity level of conversational queries can be categorized into three levels, with clear intent, as a start of a subtopic, and ambiguous ones that continue a subtopic.
\end{enumerate}

For example, in Table~\ref{tab:cast2019_q}, turn 1 starts the session with the main topic ``acid reflux'' and its intent is clear; turn 3, 5, 6 and 8 start four different subtopics; turn 7 continues the subtopic ``foods and acid reflux'' and is quite ambiguous.

In addition, it is also observed that there is a correlation of a query term's importance and the highest BM25 retrieval score of any document in the corpus to this query term. The latter is defined as:
\begin{align}
    \text{Max}\_\text{BM25}(t) &= \max_{d \in C} \{\text{BM25}(t, d) \}.
\end{align}
The intuition behind this design is that if there is a document that has very high retrieval score with a term, then the term is more likely to convey important information (which is picked up by BM25 and reflected in the BM25 score)~\cite{lin2020multi}. 

The usage of Max$\_$BM25 is correlated with the post-retrieval query difficulty prediction in ad hoc retrieval~\cite{carmel2010estimating}, though direct comparison of absolute BM25 score across different queries is less usual in IR research. Too many factors such as document length and the distribution of corpus may influence the absolute BM25 score. Nevertheless, for TREC CAsT queries and corpus, the correlation exists empirically and HQE is designed to utilize this correlation to conduct query expansion.

% \cx{To describe the term selection and query expansion determination here.}
Based on  these two set of observations on TREC CAsT data, the HQE method performs two things for query resolution. The first is to extract keywords from each query turn and maintains two set of keywords, one for main topic, the other for subtopic. The second is to determine the ambiguity level of a query turn and thus to add different groups of keywords extracted from previous turns to the query. Both utilizes the the Max$\_$BM25 score of terms and queries, as described next.


\textit{Topical Keyword Extraction.} HQE maintains two set of keywords during the conversational session: $W_\text{topic}$, the main topic keywords, and $W_\text{sub}$, the subtopic keywords. A keyword is considered as a main topic keyword if its Max$\_$BM25 score is greater than a threshold $R_\text{topic}$. Similarity, if its Max$\_$BM25 score is greater than a lower threshold $R_\text{sub}$ it is considered as a subtopic keyword.  
\begin{align}
    &t \in W_\text{topic}, & \text{ iff } \text{Max}\_\text{BM25}(t) > {R}_\text{topic} \\
    &t \in W_\text{sub} & \text{ iff } \text{Max}\_\text{BM25}(t) > {R}_\text{sub} 
\end{align}
The two thresholds $R_\text{topic}$ and $R_\text{sub}$ (    ${R}_\text{topic} > {R}_\text{sub}$) are hyperparameters to be determined, for example, by searching in the development set.




\textit{Ambiguity Level Guided Query Expansion.} The extracted main and sub topic keywords from previous turns are used to expand the current turn $i$ based on the ambiguity level of $q_i$. A query whose Max$\_$BM25 score exceeds a threshold $\eta$ is considered as non-ambiguous in HQE. Only main topic keywords are added to it. Otherwise, the sub topic keywords from previous $M$ turns are also added to it. 
\begin{align}
    q'_i &= q_i \circ S^\text{HQE}_i,\\
    S^\text{HQE}_i &= 
    \begin{cases}
    W_\text{topic}, &  \text{if}\ \text{Max}\_\text{BM25}(q_i) > \eta  , \\
    W_\text{topic} \cup  W_\text{sub}^{i-M:i-1} & \text{otherwise}.
    \end{cases}
\end{align}
The hyperparameter $M$ controls the deprecation of the subtopic keywords as the conversation may shift subtopics. It is also empirically configured using validation performance. The expansion/addition of keywords is simply concatenate the set of HQE keywords to the end of $q_i$. Then the new query $q'_i$ serves as an ad hoc query that can be used as input to standard ad hoc retrieval systems.
Note the main topic keywords are added to all queries regarding their ambiguity, including queries with clear intent where adding these keywords further emphasizes their weights in downstream retrieval\&reranking models. 



The HQE method is a rule-based classification system that first classifies terms into three categorizes, main topic, sub topic, and otherwise, and then classifies queries to two classes, ambiguous or clear intent, in order to perform conversational query expansion.
The rule-based classification is manually designed by their authors' empirical observations on the TREC CAsT data and the behavior of BM25 scores there. 

Although HQE performed well in TREC CAsT 2019, it is not as clear whether its empirical observations, as well as their underlying assumptions, are generalizable to real conversational search systems, or merely guided by some proprieties only exist in TREC CAsT datasets. Next we describe another significant approach that leverages a more standard supervised learning framework.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/QuReTeC.png}
    \caption{A example data point in the term classification task formulated in QuReTeC, from Voskarides et al.~\cite{voskarides2020query}}
    \label{fig:qeretec_eg}
\end{figure}


\textbf{Query Resolution by Supervised Term Classification.}
Another way to perform conversational query expansion is to formulate it as a supervised term classification task---to classify whether query terms in previous turns should be added to the current query~\citep{voskarides2020query}. 
This method, Query Resolution by Term Classification (QuReTeC), includes two main components: a BERT-based~\cite{devlin2018bert} binary classifier to predict whether a term in previous turns should be add to current query, and a distant supervision method that constructs term level labels to train the classifier. 
It is a simple combination the standard approach to utilize BERT in term level tasks and to construct distant supervision labels in query expansion tasks~\cite{cao2008selecting, xiong2015query}. Next we discuss the two components of this signature approach in more detail.

\textit{Expansion Term Classification with BERT.} QuReTeC uses BERT as the classification function $g()$ in Eq.~\ref{eq:expterm_classification}. As illustrated in Figure~\ref{fig:qeretec_eg}, the input to its BERT model is the concatenation of all previous queries with the current query; the BERT is used to predict a binary label on each term in previous queries.

Specifically, QuReTeC first uses BERT to generate the contextualized representation for each term $t_k^j$ in previous queries:
\begin{align}
    \mathbf{H} = \text{BERT}(\text{[CLS]}q_1 \circ...\circ q_j \circ... \text{[SEP]} \circ q_i),
\end{align}
where $\circ$ is the concatenation operation, [CLS] and [SEP] are the special tokens, and $\bf{H}$ is the contextualized representation provided by the last transformer layer in BERT.

Let $\bf{h}_j^k$ be the corresponding vector in $\bf{H}$, QuReTeC uses a linear layer with sigmoid activation to predict the binary classification labels:
\begin{align}
    g(t_k^j; q_{1:i}) &= \text{Sigmoid}(\text{Linear}(\mathbf{h}_k^j)).
\end{align}

\textit{Training with Term-Level Distant Supervision.}
The simplest way to train the term level classifier is to use term level labels, e.g., a binary label on each term on whether it is a good expansion term, and fine-tune the BERT model with standard classification loss. 
Such term level labels are in general not available in search and often derived from relevance labels, for example, by the influences on final ranking accuracy when the term is used to expand the query~\cite{cao2008selecting}. This is often referred to as distant supervision and widely used in various tasks~\cite{mintz2009distant}.

QuReTeC leverages the relevant documents $d^+$ to generate the distant term level labels. It labels a term as positive expansion term if it appears in a query's relevant document and also in previous queries, but not appear in the current query:
\begin{align}
    S^* &= terms(d^+_i) \cap terms(q_{1:i-1}) \setminus terms(q_i). \label{eq:qeretec_sup}
\end{align}
Here $terms()$ denote all the terms in the query or document. 

Eq.~\ref{eq:qeretec_sup} selects terms that 1) appears in the relevant document but not in the query and 2) also appears in previous query turns.
The first is intuitive as such as term is likely to benefit ranking accuracy as it improves the term overlap between query and relevant document. It is similar to the distant supervision approach used in ad hoc query expansion~\cite{cao2008selecting}.
The second assumption restricts the expansion term to only from previous query rounds as it is the candidate set the term classification model works with. In CAsT 2009 data, they observe that the majority of new terms in the oracle manual de-contextualized queries are from previous query turns~\cite{voskarides2020query}. Whether this assumption and observation hold for other conversational search benchmarks and in real scenarios is another question to ask when applying conversational query expansion techniques on those scenarios.




\subsection{Conversational Query Rewriting}
Another technical choice for contextual query understanding is to leverage natural language generation (NLG) models to directly rewrite the conversational turns into a de-contextualized, single-turn, natural language query.
% Besides adding expansion terms to conversational queries, another approach to resolve the contextual dependency challenge emerged in TREC CAsT 2019 is to directly rewrite a de-contextualized query using natural language generation (NLG) methods~\cite{vakulenko2020question}. 
In the rest of this section, we first describe the formulation of \textit{conversational query rewriting}, first by \citet{vakulenko2021question}, and then how to better train the query rewriter with weak supervision signals.


\textbf{Conversational Query Rewriter.} In TREC CAsT 2019, Vakulenko et al.  presented a simple and effective way to utilize NLG models in conversational query understanding~\cite{cast2019overview, vakulenko2021question}. They use an NLG model, ``query rewriter'', to rewrite the conversational query to a de-contextualized ad hoc query using a NLG model:
\begin{align}
    \{q_1,...,q_{i-1}\}, q_i \xrightarrow{\text{NLG}} q'_i,
\end{align}
where the rewritten query $q'_i$ aims to approximate the oracle manual de-contextualized query $q^*_i$.

More specifically, they fine-tune GPT-2, the pretrained unidirectional transformer decoder model~\cite{radford2019language}, as their query rewriter:
\begin{align}
    q'_i &= \text{GPT-2}(\text{[CLS]} q_1 \circ \text{[SEP]}....\text{[SEP]}q_{i}  \circ \text{[GO]}).    
\end{align}
The GPT-2 based query rewriter takes the input of all queries from previous turn and concatenate them with the current query, uses a special token ``[GO]'' to mark the end of contextualized input, and directly generates a natural language query $q'_i$ from there.  The generating of the new query can use any standard decoding approach in NLG~\cite{reiter1997building}. In conversational query rewriting, simple decoding strategies such as greedy search and beam search are often sufficient.


To fine-tune the rewriter, one can use the manually query rewrites $q^*$ as the ground truth labels and trains the GPT-2 model following standard approaches NLG, such as teacher forcing~\cite{williams1989learning}. 
The TREC CAsT datasets only have hundreds of such manual query rewrites, raising concerns whether such a small amount training data would lead to overfitting with deep neural networks like GPT-2. A common approach is to leverage the crowd sourced query rewrites in CANARD~\cite{elgohary2019canard} as additional fine-tuning data. 

A vanilla adaptation of GPT-2 in conversational query understanding, this conversational query rewriter is simple and effective. It lead to one of the best performance in TREC CAsT 2019~\cite{cast2019overview} and later became a standard solution adopted by many participants in TREC CAsT 2020~\cite{cast2020overview}. It is also easy to plug or combine the query rewriter with other conversational query understanding approaches, for example, using the rewritten query as another query field~\cite{lin2020multi}.

\begin{figure}
     \centering
          \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Converter.png}
         \caption{Training Data Generator}
         \label{fig:conv_converter}
     \end{subfigure}
          \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/rewriter.png}
         \caption{Conversational Query Rewriter}
         \label{fig:conv_rewriter}
     \end{subfigure}

     \caption{The illustration of self-leaning framework in conversational query rewriting. A GPT-2 converter is first used to convert ad-hoc non-contextualized query sessions into conversational search sessions (a), which are used to fine-tune the GPT-2 rewriter to reconstruct the non-contextualized queries from conversational queries (b). }
     \label{fig:conv_selflearn}
\end{figure}
    

\textbf{Few-Shot Learning of the Rewriter.} It is not always the case that a large amount of manually rewritten de-contextualized queries like CANARD is available in conversational search. As a new application,  a lot of conversational search scenarios are effectively ``few-shot'', as not many user feedback signals nor manual annotations are available to fully-supervise the query rewriter. To address the concern that lacking such high quantity training data may prohibit effective training of the query rewriter, Yu et al.~\cite{Yu2020Rewriter} build a self-learning framework that leverages ad hoc search sessions to construct weak-supervision signal for the rewriter.
The ad hoc search sessions are more likely to be available in mass quantity as ad hoc search is a more mature application than conversational search.

The idea of Yu et al.~\cite{Yu2020Rewriter} is to use a generative converter that learns to convert ad hoc search sessions to conversational formats. Then the converted ad hoc-conversational session pairs can be used as additional weak supervision signals to train the query rewriter. The two components are illustrated in Figure~\ref{fig:conv_selflearn}. In addition to a small amount of conversational search sessions $\{q_1,...q_i...,q_n\}$ and their de-contextualized targets $\{q^*_1,...q^*_i...,q^*_n\}$, it uses another set of ad hoc search sessions $\{\bar{q}^*_1,...\bar{q}^*_i...,\bar{q}^*_n\}$, which is at a much larger amount, and performs the following steps.

\textit{Step 1, Fine-tune converter.} It first uses a small amount of conversational queries and their annotations to train a GPT-2 based converter:
\begin{align}
     \{q^*_1,...q^*_i\} \xrightarrow[\text{Train}]{\text{GPT-2 Converter}} q_i.
\end{align}
The converter takes the input of manual de-contextualized queries and learns to convert them back to the raw conversational queries.

\textit{Step 2, Convert ad hoc sessions to conversational-alike sessions.} It then uses the trained GPT-2 converter to convert on ad hoc search sessions to conversational-alike sessions. 
\begin{align}
     \{\bar{q}^*_1,...\bar{q}^*_i\} \xrightarrow[\text{Inference}]{\text{GPT-2 Converter}} \bar{q}_i.
\end{align}
The ad hoc search sessions are available at the millions or billions in commercial search. In Yu et al.~\cite{Yu2020Rewriter} they use the MS MARCO syntactic sessions which are MARCO queries ``glued'' together using embeddings~\cite{zhang2019generic}.

\textit{Step 3, Train query rewriter with converted session pairs.} The converted session pairs are then used to fine-tune the GPT-2 rewriter:
\begin{align}
    \{\bar{q}_1,...\bar{q}_i\} \xrightarrow[\text{Train}]{\text{GPT-2 Rewriter}} \bar{q}^*_i.
\end{align}
The fine-tuned GPT-2 rewriter are then used to rewrite actual conversational search queries to their corresponding de-contextualized ad hoc formats.

The key assumption behind this self-learning framework is that, in step one, it is easier to train a converter that learns to omit information from an ad hoc query using session context, than to train a rewriter that learns to recover the omitted information. Empirically, Yu et al.~\cite{Yu2020Rewriter} shows this self-learning approach can significantly boost the performance of the same GPT-2 query rewriter on TREC CAsT benchmarks.






\textbf{Recap.} 
Now we have discussed various approaches for contextual query understanding, we can put them together with an ad hoc search system for an instantiation of the sparse conversational search system in Figure~\ref{fig:convsearch_arch}:
\begin{align*}
    & \{q_1,...,q_{i-1}\}, q_i \xrightarrow[\text{Expansion/Rewriting}]{\text{Conversational Query}} q'_i,  & \text{Contextual Query Understanding} \\
    & d \xrightarrow[\text{Document Expansion}]{\text{Bag of Words}} d', & \text{Ad hoc Document Understanding} \\
    & D_\text{BM25}^q = \text{Top}_k \text{BM25}(q'_i, d').  & \text{BM25 first stage retrieval}, \\
    & f(q'_i, d') = \text{Linear} (\text{BERT}_\text{CAT}(\text{[CLS]} \circ q \circ \text{[SEP]})). & \text{BERT Ranker}
\end{align*}
The documents, ordered by their ranking score $f(q'_i, d')$, form the relevant document output of the conversational search system. 






==> chapter_cir/06_dense.tex <==
\section{Dense Conversational Search Approaches}
\label{sec:ConvDR}

In previous section, we discussed the vocabulary mismatch being an intrinsic challenge of sparse term based retrieval systems. 
The expansion techniques can reduce the lexicon gaps between query and relevant documents, but the fundamental challenges that yield the vocabulary mismatch problem still remain, for example, language variety, independent bag-of-words assumption,  sparse discrete representation space, et cetera.

Besides enriching the term-based representations in search, there have been many other attempts to solve the vocabulary mismatch problem.
One direction is to reduce the criteria of vocabulary match from exact to soft match. For example, the translation model framework~\cite{berger1999information} counts for the relatedness between two distinct terms in query and documents. The relatedness or soft match score between two terms is calculated based on their correlation statistics in the corpus~\cite{berger1999information} or learned end-to-end in Neural Information Retrieval~\cite{mitra2018introduction, xiong2017knrm}.
Another direction, \textit{representation learning}, is to directly learn a new representation space that captures the semantic matches between queries and documents.
This dates back to at least in the 90s where dimension reduction techniques were used to index documents by latent semantic analyses~\cite{deerwester1990indexing}.  


With the resurrection of neural networks and the revolution of pretrained language models, representation learning techniques start to show remarkable progress in addressing the vocabulary mismatch problem for information retrieval. 
It is effective to learn a continuous representation space for the natural language queries and documents and match them directly using their dense embedding vectors. The technique, coined as ``dense retrieval'', has been widely studied since 2019 and advanced the retrieval accuracy of many ad hoc and conversational search benchmarks. In this section, we first present the preliminary of dense retrieval (Sec.~\ref{sec:DR_prelim}).  Then we introduce how to perform dense retrieval in conversational search (Sec.~\ref{sec:conv_dr}) and how to train dense retrieval models in few-shot scenarios (Sec.~\ref{sec:fewshot_conv_dr}).




% \begin{figure}[t]
%  \centering
%           \begin{subfigure}[t]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{fig/concat.pdf}
%          \caption{Concatenation ($\text{BERT}_\text{CAT}$).}
%          \label{fig:concate}
%      \end{subfigure}
%           \hfill
%      \begin{subfigure}[t]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{fig/siamese.pdf}
%          \caption{Dual-Encoder  ($\text{BERT}_\text{ENC}$).}
%          \label{fig:Siamese}
%      \end{subfigure}
% \caption{Two ways to leverage pretrained transformers in information: Concatenation which is used in reranking and Siamese which is used in retrieval.}
% \label{fig:plm_usage}
% \end{figure}

\subsection{Preliminary on Dense Retrieval}
\label{sec:DR_prelim}

% In this part we discuss some backgrounds of dense retrieval (DR). 
As a emerging and rapid developing topic, we mainly cover a basic DR setup with pretrained language models, the challenge in its early development and the solutions recently developed in 2020. We encourage readers to check recent literature for more up-to-date progress if interested.


\textbf{Dense Retrieval Setup.} 
% Dense retrieval performs first stage retrieval using the dual encoder setup described in Section~\ref{sec:cir_preliminary}. Itf irst 
As discussed earlier, the first stage retrieval can be viewed as to construct a scoring function between query and document:
\begin{align}
    f(q, d) &= \text{sim}(\mathbf{q}, \mathbf{d}),
\end{align}
where $\mathbf{q}$ and $\mathbf{d}$ are the vector representation of the query and document and sim() is the similarity function to match two vectors.
The first stage retrieval requires the similarity function to support efficient look up of top K most similar documents for a query in a large corpus. 

In sparse retrieval systems, $\mathbf{q}$ and $\mathbf{d}$ are sparse vectors, such as bag-of-words, and sim() is frequency based functions like BM25. 
In dense retrieval, the representation of query and documents are learned continuous vectors (``embeddings''):
\begin{align}
    \mathbf{q} &= g_q(q);  &   \mathbf{d} &= g_d(d).
\end{align}
The two functions, $g_q$ and $g_d$, are often referred to encoders. They map the natural language queries and documents to embeddings which are continuous vectors, often in hundreds of dimensions. Retrieval with learned embeddings is thus referred as ``dense retrieval'' or ``latent retrieval'', to distinguish with sparse retrieval which operates with sparse and explicit bag-of-words vectors. 

Efficient retrieval of top K documents in the embedding space, i.e., finding the K nearest neighbors of a given query embedding, is a different task from in the sparse space. Different data structure and infrastructure are needed. It is also common to trade-off the exactness of top K neighbors for efficiency, using approximate nearest neighbor (ANN) search. The search can also use speed up from GPUs infrastructures and batching. For more details about the available toolkits and algorithms in efficient nearest neighbor search, we refer readers to the ann-benchmark work\footnote{http://ann-benchmarks.com/} as the entry point for references~\cite{aumuller2017ann}. 


The choice of the similarity function in DR then depends on whether the metric is supported in the nearest neighbor search infrastructure, for example, your choice of ANN search toolkit. Most publicly available toolkits support maximum inner product search, L2 distance, and cosine distance, for example, in the FAISS library used in several papers to be discussed in this section~\cite{FAISS}.


\textbf{Dense Retrieval with Pretrained Transformers.} 
A successful way to instantiate DR is to use pretrained transformers in the dual-encoder formulation~\cite{lee2019latent}, as discussed in Section~\ref{sec:cir_preliminary}.:
\begin{align}
    f(q,d) &= g(q) \cdot g(d) \\
    g(q); g(d) &= \text{BERT}(q); \text{BERT}(d).
\end{align}
We use $\text{BERT}(x)$ to denote the BERT based representation of a text sequence $x$, which is often the [CLS] embedding of the last layer. The average of token embeddings of BERT's last layer can also be used. 
It is also found that though it is not necessary to use the same models in the query and document encoders, using the same model with shared parameter weights on two sides works well empirically. 

\textbf{Challenges in Dense Retrieval Models}
You may notice the use of BERT in dense retrieval is quite different from in reranking.  Putting the reranking and retrieval function with BERT together:
\begin{align}
    f_\text{rerank} &= \text{Linear} (\text{BERT}(q \circ d)), \\
    f_\text{retrieval} &=  \text{BERT}(q) \cdot \text{BERT}(d),
\end{align}
we can see that in reranking the BERT model is applied on the concatenation of query-document pairs, while in retrieval the query and document are first encoded by BERT \textit{individually} and then matched using simple similarity functions. 

As illustrate in Figure~\ref{fig:plm_usage}, the different ways of using BERT in reranking and retrieval are due to different capacity-efficiency trade-off at different stages. In reranking, the candidate documents to rerank is pre-given, e.g., from retrieval, and are in the order of hundreds or thousands. It is possible to enumerate BERT on all q-d pairs in reranking. At the same time, feeding the concatenation of q-d pairs to BERT enable it to explicitly capture the term level matches between query and documents, as its self-attention mechanism is applied on all q-d term pairs.
The capacity of explicit term-level matching makes $\text{BERT}_\text{CAT}$ a more effective model than dual encoder although also less efficient~\citep{mitra2018introduction, xiong2017knrm}.

In comparison, $\text{BERT}_\text{CAT}$ is infeasible in dense retrieval as the candidate documents to score are the entire corpus. It is infeasible to enumerate all documents for each query in first stage retrieval (unless the corpus is very small, making it no longer a retrieval task).
It is usually a necessity to encoder the query and document separately using the dual-encoder architecture ($\text{BERT}_\text{ENC}$) to support first stage retrieval. 

Modeling search relevance with $\text{BERT}_\text{ENC}$ is more difficult than with $\text{BERT}_\text{CAT}$. All the information of a query or a document is compressed into one or a few embedding vectors and the relevance match is done by metrics as simple as dot product. Even capturing exact term match with dual-encoder is not as trivial as in $\text{BERT}_\text{CAT}$ where the attention mechanism can easily cover exact match.

Another difficulty in dense retrieval is its large decision space. For each query, the DR model is to determine the most relevant documents from the entire corpus, e.g., millions or billions of documents, while in reranking the ranking model only needs to distinguish relevant documents from hundreds or thousands of candidate documents that are already filtered by previous stages. 
% challenge and difference with LeToR
These obstacles make dense retrieval a challenging task. Earlier explorations of deep learning technique in retrieval, also referred to ``representation-based'' Neu-IR models, often found underwhelming performances far behind simple BM25, even in web search where sufficient relevant training signals are available~\cite{mitra2018introduction}. 


\textbf{Training Strategies and Negative Sampling for Dense Retrieval.}
Recent research identified the training strategy, specifically, the construction of negative training instances, as one of the key challenges in the early stage of dense retrieval. 
Next we first describe the formulation of DR training using a typical learning to rank setting, which leads to the challenges in finding proper negatives. Then we present two recent approaches that construct better negatives and elevate dense retrieval to outperform traditional sparse retrieval in answer passage retrieval and web search benchmarks~\cite{karpukhin2020dense, xiong2020approximate}.
% Various approaches have been proposed to 

% ways to train it
In standard learning to rank~\cite{liu2009learning}, 
the ranking model $f()$ is trained with a set of relevant document $D^+$ and irrelevant document $D^-$ for each query q, for example, using the following loss function:
\begin{align}
    \theta^*= \text{argmin}_\theta \sum_{q} \sum_{d^+ \in D^+} \sum_{d^- \in D^-} l(f(q, d^+), f(q, d^-)),
\end{align}
to find the optimal parameter $\theta^*$. The loss function $l()$ can be simple classification loss, e.g., binary cross entropy (BCE) loss to learn to classify whether a document is relevant or not and train, or other standard learning to rank losses~\cite{liu2009learning}.

In reranking, choosing $D^+$ and $D^-$ is intuitive: Documents labeled relevant or clicked by users are $D^+$ and other candidate documents to rerank (e.g., those top retrieved ones) form the negatives $D^-$. These are the same as the candidate documents to be reranked by the model at testing time and have been widely used as standard in LeToR.

In first stage retrieval, the choice of positives $D^+$ is the same,
but choosing proper training negatives is challenging. The reason is that, at retrieval, the model is asked to separate relevant documents from the rest of the entire corpus ($D^- = C \setminus D^+$). This easily leads to millions of negative instances that have to be sampled during training:
\begin{align}
    \theta ^* &= \text{argmin}_\theta \sum_{q} \sum_{d^+ \in D^+} \sum_{d^- \in \hat{D}^-} l(f(q, d^+), f(q, d^-)),
\end{align}

Recent research found that using standard sampling to construct the negative documents $\hat{D}^-$, for example, in-batch randoms, does not train effective dense retrieval models~\cite{karpukhin2020dense}. Empirically, randomly sampled negatives are often too trivial and do no push the model much; theoretically, they yield scholastic gradients with high variances which hinder model convergence~\cite{xiong2020approximate}.

One way to improve the negative sampling is to leverage sparse term-based ranking models to produce challenge negatives, for example, by sampling from the top ranked irrelevant documents by a sparse search system:
\begin{align}
    \hat{D}^- &= D^-_\text{random} \cup D^-_{f_\text{sparse}}.
\end{align}
We use $D^-_\text{random}$ to denote the randomly sampled negatives and $D^-_{f_\text{sparse}}$ to note the negatives sampled from the top ranked documents in a sparse ranking system $f_\text{sparse}$. The sparse ranking model used to construct negatives can be BM25~\citep{karpukhin2020dense} or even a BERT-based reranker on top of BM25~\cite{ding2020rocketqa}.

Piggybacking sparse retrieval systems' output provides a head start for dense retrieval but also raises concerns whether DR models alone are able to outperform sparse retrieval models~\cite{luan2020sparsedense}. Using the sparse model to provide training signals may boost dense retrieval to mimic sparse retrieval, but not necessarily to compensate sparse retrieval not overcome their fundamental limitations.

One research front to address this concern is to directly train dense retrieval using negatives from the DR model itself during learning. 
One straightforward solution is to directly samples negative documents using the being optimized DR model itself~\cite{xiong2020approximate} :
\begin{align}
\hat{D}^- &= D^-_{f_\text{DR}}.
\end{align}
The negatives are sampled from the top K retrieved documents from the DR model $f_\text{DR}$. As a result, the distribution of the negatives seen by the DR model during training are aligned with the negatives to be distinguished at testing. 

Xiong et al.~\cite{xiong2020approximate} provides theoretical analyses on the impact of negative sampling in dense retrieval training using the variance reduction and negative sampling framework~\cite{alain2015variance, katharopoulos2018not}. They show that sampling negatives randomly is unlikely an effective importance sampling strategy and often yields inefficient learning convergence. 

% \begin{enumerate}
%     \item Most documents in a corpus are trivially irrelevant to a query and the main challenge in retrieval is to distinguish a small amount of hard negatives.
%     \item Dense retrieval models, operating in a continuous space, behave dramatically different from classic sparse retrieval systems, i.e., the top ranked documents from two pipelines have limited overlaps.
% \end{enumerate}
% Both properties are empirically verifiable in common retrieval benchmarks. For the detailed theoretical proof we refer readers to Xiong el at.~\cite{xiong2020approximate}.

Sampling negatives from the up-to-date DR model during training is challenging as the DR model is updated in each mini-batch.
% and it is often infeasible to use the most updated DR model to retrieve negative documents, which would require refreshing the document encoding of the entire corpus. Xiong et al. uses 
% There are various ways to trade off the freshness of DR models used in sampling for efficiency. 
Xiong et al. uses the asynchronous approach developed by \citet{guu2020realm}. It maintains another set of GPUs to recalculate the document encodings of the corpus, using a previous checkpoint of the being trained DR model, and refreshes the ANN index for negative sampling only when the inference is finished. 

In the rest of this section, we describe how to build conversational search systems upon dense retrieval models.
Unless specified, there is no restrict of which DR model to use as the building block for the conversational search system. One can choose the newest state-of-the-art DR model and benefit from the development of dense retrieval.

\subsection{Conversational Dense Retrieval}
\label{sec:conv_dr}

% use DR as an ad hoc system

A straightforward way to leverage DR models in a conversational search system is to replace the sparse ad hoc retrieval module with as dense retrieval system.
For example, in the system described in Sec.~\ref{sec:convsearch_bow}, after obtaining a reformulated ad hoc query $q'$, either by conversational query expansion or rewriting, we can treat $q'$ as an ad hoc query and feed it through a dense retrieval system for first stage retrieval. Assuming the DR system is more effective or compensates a sparse retrieval system, this often lead to improved final conversational search accuracy~\cite{yu2021convdr}.


% problems of this query reformulation + ad hoc framework
    % hard to obtain intemidate labels
    % hard to train the retriever with QR, discrete decision space, hard to train a QR with retrieval loss
This approach, however, faces the same challenges in the query reformulation part as discussed in last section. The query reformulation is a discrete process that is hard to be trained directly from the relevance labels. The reformulation models, NLG or term classification, are often trained with intermediate query level labels that are harder to obtain, compared to relevance labels. 
    
    \begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/ConvDR.png}
    \caption{An illustration of a standard conversational dense retrieval system used in recent research~\cite{qu2020orqa, yu2021convdr}. The figure is from Yu et al.~\cite{yu2021convdr}.} \label{fig:convdr}
\end{figure}
    

% advantage of DR in this formulation    
    % with DR, it is no need to have an explicit natural language query or bag-of-words, all it is needed is to have an embedding that captures user's information need
    % DR is fully trainable
On the other hand, different from sparse retrieval,
 dense retrieval systems do not require an explicit reformulated query $q'$. All it needs is an embedding vector $\mathbf{q}$ that represents user's information needs, no matter reflected in one ad hoc query or a multi-turn conversation. 
At the same time, dense retrieval models are fully-trainable, making it easier to learn embeddings for the conversational rounds. 

Qu et al.~\cite{qu2020orqa} is among the first to explore a such conversational dense retrieval (ConvDR) model that directly learns a contextualized encoding for a conversational round in the dense retrieval setting. At the $k$-th turn, the conversational DR model is formulate as:
\begin{align}
    f(q, d) &= \mathbf{q} \cdot \mathbf{d}, \\
    \mathbf{q} &= g_q(q) = \text{BERT}(\text{[CLS]} q_1 \circ \text{[SEP]}....\text{[SEP]}q_{k} \text{[SEP]}), \\
    \mathbf{d} &= g_d(d) =  \text{BERT}(\text{[CLS]} d \circ \text{[SEP]}).
\end{align}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/ConvDRTrain.png}
    \caption{The teacher-student framework to train a ConvDR model using an ad hoc teacher with limited supervision signals~\cite{yu2021convdr}.} \label{fig:convdrtrain}
\end{figure}


Instead of an ad hoc or a reformulated query, here the query encoder $g_q()$ takes all previous conversational rounds (or plus responses if needed) as the input and aims to produce a contextualized embedding $\mathbf{q}$ that captures user's information needs reflected up to the current conversation turn.
The system is illustrated in Figure~\ref{fig:convdr}.

Compared to the conversational query reformulation solution in sparse retrieval, this conversational DR 
It has the access to the same context information as a conversational query reformulation model in the sparse retrieval setting,
but can be trained end-to-end directly using the relevant label.
The full system is trainable, for example, using the following ranking loss per query turn:
\begin{equation}\label{eq:rank_loss}
    \mathcal{L}_{\text{Rank}}=-\sum_{d^+ \in D^+}\log \frac{\exp \left(\mathbf{q}_k \cdot \mathbf{d}^+ \right)}{\exp \left(\mathbf{q}_k \cdot \mathbf{d}^+\right)+\sum\limits_{d^{-} \in \hat{D}^{-}} \exp \left(\mathbf{q}_k \cdot \mathbf{d}^-\right)},
\end{equation}
with relevant documents $D^+$ and constructed irrelevant documents $\hat{D}^-$.

Qu et al.~\cite{qu2020orqa} demonstrate the effectiveness of this ConvDR solution in a conversational open retrieval setting when there are sufficient relevant labels to fully-supervise the ConvDR model.




% leads to the conver dr set up first proposed in Qu ORQAin the conversaitonal QA setting where a lot of supervision signal data is available by answer distant supervision


% first attempt \cite{qu2020orqa}


\subsection{Training Strategies in Few-shot Settings}
\label{sec:fewshot_conv_dr}

As discussed in Sec.~\ref{sec:DR_prelim}, training a dense retrieval model for ad hoc search is a non-trivial task even with sufficient relevance training signals. 
Intuitively, it is more challenging to train a ConvDR model because 1) training data in conversational search scenarios are often more limited; 2) representing user's search intents behind a complex multi-turn conversation is more complicated or at least less-understood than encoding an ad hoc query. 
This makes training a ConvDR model a more difficulty task especially in few-shot settings.

In the rest of this section we discuss a recent approach that trains ConvDR models in few-shot settings where relevance labels are limited~\cite{yu2021convdr}.
% few-shot learning approach for ConvDR using an ad hoc DR model as the teacher~\cite{yu2021convdr} 
It uses a fully-supervised ad hoc dense retriever as the teacher and distills the representation model to ConvDR with the help of a small amount of manually de-contextualized queries.

More specifically, given a small amount of (e.g., in hundreds) conversational search turns $\tau=\{q_1,...,q_n\}$ with labeled relevance documents and manual de-contextualized query rewrites $q^*$, Yu et al.~\cite{yu2021convdr} assumes the following properties in the scenario: 1) There exists a fully-supervised ad hoc dense retriever $f_\text{DR}$ that effective encodes the de-contextualized ad hoc query $q^*$; 2) The dense representation of document in the corpus is universal across different search formats, that the  information of a document is the same, whether it serves ad hoc or conversational search.
Both properties are likely satisfied in domains where exist a mature ad hoc search system, for example, in web search and the TREC CAsT setting~\cite{yu2021convdr}.

Within these assumptions, we can reuse the document encoder learned for ad hoc search in conversational search, and train the conversational query encoder by distillation from the encodings of de-contextualized query from the ad hoc DR model. Yu et al.~\cite{yu2021convdr} shows this can be achieved by a mean square error (MSE) loss that minimizes the per dimension encoding difference:
\begin{align}
    \mathcal{L}_{\text{KD}} &= \text{MSE}(\mathbf{q}_k, \text{ANCE}({q}^*_k)),  \label{eq:KD_loss} \\
    \mathbf{q}_k &= \text{ConvDR}(q_{1:k}), \\
    g_\text{ConvDR}(q_{1:k}) &= \text{BERT}(\text{[CLS]} \circ q_1 \circ \text{[SEP]}....\text{[SEP]} \circ q_{k} \circ\text{[SEP]}).
\end{align}
It trains the BERT-based ConvDR encoder $g_\text{ConvDR}()$ to mimic the encoding $\text{ANCE}({q}^*_k))$ of ad hoc query $q^*_k$ from the DR teacher's encoder, in this case, ANCE. 
At the same time, the document encoder is kept the same with the ad hoc DR model:
\begin{align}
     g_\text{ConvDR}(d) &= \text{ANCE}(d).
\end{align}

As illustrated in Fig.~\ref{fig:convdrtrain}, the knowledge distillation loss can be combined with the (few-shot) ranking loss to boost the ConvDR model training. The same few-shot strategy can also be used to obtain a contextualized BERT ranker:
\begin{align}
    f(q_{1:k}, d) &= \text{Linear} ( \text{BERT}(\text{[CLS]} q_{1:k} \circ  \text{[SEP]} \circ d)), \\
    q_{1:k} &= q_1 \circ \text{[SEP]} \circ ... \text{[SEP]} \circ q_k.
\end{align}
It directly takes raw conversational turns and learns to rank the documents for them.

\textbf{Recap.} Putting everything together leads to the following instantiation of conversational search.
\begin{align*}
    & \bs{q}_i = \text{ConvDR} (q_1,...,q_i); & \text{Contextual Query Understanding} \\
    & \bs{d} = g_\text{ad hoc} (d); & \text{Document Understanding}; \\
    & D^q_\text{DR} = \text{KNN}_{\bs(d)}(\text{sim}(\bs(q)_i, \cdot)); & \text{KNN/ANN Retrieval} \\
    & f(q_i, d) = \text{Linear} ( \text{BERT}(\text{[CLS]} q_{1:k} \circ  \text{[SEP]} \circ d)). & \text{BERT Ranker}.
\end{align*}
The ranked documents are the output of the conversational search system, either directly served to the user or passed to latter components in the CIR system for more fine-grained responses.




















==> chapter_cir/07_challenges.tex <==



\section{Challenges and Future Research}
\JG{move this section to the last chapter of the book.}

While the recent progress (up to December, 2021) has pictured a promising future of conversational search and laid a solid foundation for the future development,    
it is unarguable that the field is still at its infant stage. 
A conversational search engine that goes beyond ad hoc search  to effectively meet users' information needs of wide diversity and complexity is yet to be developed. 
This section presents some of the most important challenges yet to be addressed.
%In the last section of this chapter, we discuss some known challenges in conversational search. We note that as a premature topic with rapid development, new challenges  may occur and existing ones may be solved with new techniques straightforwardly.

% reusable benchmarks for interactive search
\paragraph{Evaluation.}
%{Creating Robust and Reusable Benchmarks.}
The interactive nature of conversational search makes it challenging to develop robust and reusable evaluation methods.
%As naturally the user behavior depends on the system response, the conversation trajectory is a result of user-system interaction. 
Although off-policy evaluation based on pre-collected datasets is widely used to measure the individual CIR modules, such as the modules of query understanding, document retrieval and ranking, as described in this chapter, it is insufficient to measure how effective a system \emph{interacts} with users to accomplish a search task. 
% Offline evaluation with a fixed dataset often has to restrict to a pre-given, still, conversational trajectory that only covers one potential conversational path in the space. 
% It is hard to capture all the aspects and user intern space using static offline benchmarks.
%On the other hand, it is crucial to have usable offline benchmarks to facilitate rapid development of new methods.
On the other hand, online system evaluation based on simulated users and A/B test are too costly to perform frequently, especially at the stage of research exploration. 
Thus, how to leverage different evaluation methods to seek the best tradeoff between low cost and high reliablity is a real challenge not only for CIR, but also for all other interactive AI systems.
%This is a shared challenge with other interactive IR systems. How to balance the reusability and the realisticness when designing benchmarks for conversational search is a challenging but important task---A model is only as good as its evaluation benchmark can reflect.

\paragraph{Putting Pieces Together.}
While there are many studies on developing individual CIR components, there is few systematic research on how to piece together these components to build an effective CIR system, which requires the development of a global dialog manager which maintains the dialog state and determine how to respond a user input. Such a dialog manager needs to be optimized for a long-term reward, such as increasing the number of active users in three months. 

\paragraph{Building a CIR ecosystem.}
how to get the snowball rolling? 
Deploy primary CIR systems, get user logs, improve CIR systems...  XiaoIce is a good example.

\paragraph{Ethic concerns and responsible AI}

\paragraph{Continual learning.}
from a static setting to a dynamic setting...

\paragraph{Modeling Long Dialog History.}
For many complex search tasks, such as learning and investigating searches, a user may have to work with the CIR system for days or weeks, generating very long conversation sessions. How to capture these long dialog context for response generation remains an open challenge. For example, the BERT-based retrieval model described in Section~\ref{sec:conv_dense_retrieval} can only take a few thousand tokens as input. Thus, recent studies~\citep[e.g.,][]{xu2021beyond} start to explore the use of external memory to capture long dialog context for response generation.  

%Almost all query understanding solutions discussed in this chapter leverages a pre-trained model, many of them BERT/RoBERTa, to model the context in previous rounds.
%Their self-attention mechanism is remarkably effective in capturing salient context by taking the input of all previous rounds' queries in concatenation.
%However, when the conversation become longer, or more critically, more information from previous system responses are required, the contexts will exceed the maximum sequence length of a pretrained model and can not be captured by the self-attention of, for example, one BERT-based model.
%Recent research has explored solutions such as filtering down the candidate contexts to BERT's maximum length, or leveraging hierarchical models that combine multiple BERTs together, but they are not as effective as simply feeding everything to one pretrained transformer when feasible.
%It is unclear whether dedicated approaches are required to model more complicated context in conversational search, or the pretrained models on long-form texts will become efficient and effective enough for conversational search.
% so that we can keep using them off-the-shelf.

% how much can we piggybacking ad hoc search


%\textbf{When Piggybacking Ad Hoc Search No Longer Suffice.}

%At its early stage, it makes sense for a conversational search system to piggyback from an ad hoc search system as the teacher. However, mimicking ad hoc search is not the goal of conversational search. To expand the frontier of information retrieval, eventually conversational search systems will have to leverage the unique advantages of the conversational interaction and provide users better information access. To go there we may need research progresses in multiple fronts and from multiple disciplines, perhaps also practices with real conversational search products, and an ecosystem of research, production, and user base.


%\textbf{Roles, Integration, and Evaluation in a Conversational Assistant.}
%In real scenarios, conversational search often serves as a part of a conversational assistant. For example, in mobile devices there is often one unified entry point for the user to initial interaction, which is often referred to as a conversational/personal assistant. There conversational search can serve as a vertical or also a fall-back strategy when other functionality fails. Recently, a decent amount of research progresses have been made in each component of a such federated system, for example, task-oriented dialog, chit-chat, conversational search, recommendation, system initiatives, and dialog management. On the other hand, as the research on many of those components is in the early stage, there has not been much study on how to put together for the best end user experience. What is the best end user experience for conversational assistant is an open question itself.

%\cx{To write some general recap when all chapters are finished.}












==> chapter_iir/01_clariq.tex <==

\section{Ask Clarifying Questions}
The conversational interfaces of CIR, such as mobile screens and speech interfaces, present the retrieved result in a very concise form e.g., a direct answer to a user query instead of a rich SERP.
This limits the use of “fall back” strategies used by web search systems, e.g., diversification and federated search, and presents a stronger requirement of correctly understanding user’s information needs and a higher precision of the retrieved results.
On the other hand, the interactive nature of CIR also provides new opportunities for the system to directly ask users to clarify what they want. As shown in a user study conducted by Zamani et al.~\cite{zamani2020generating} in the Bing platform, users found an explicitly clarification function (e.g., Figure~\ref{fig:clariQplane}) convenient, time-saving, and help them shape their information needs.
Their online A/B test with Bing users also show that users prefer natural language clarification questions, rather than a purely functional static statement like ``select one to refine your search''.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{chapter_iir/clariq_bing.png}
    \caption{The clarification question function in Bing web search, as of June 2021.} \label{fig:clariQplane}
\end{figure}

In this section, we first describe the tasks required by this new functionality in conversational IR. Then we present the benchmarks curated in recent research, a typical modeling solution for these tasks, and the evaluation methodologies developed to evaluate this new function.




\subsection{Tasks}
The clarification question functionality in conversational search requires the system to perform two tasks. The first task, \textit{Unclear Question Identification}, is to identify when to ask clarification questions. The second task, \textit{Clarification Ranking/Generation}, is to determine what questions to ask. 


\textbf{Unclear Question Identification} can be considered as a sub-task of the dialog management module, as we discussed in Chapter~\ref{sec:dialog-policy}.

\begin{task}
\textit{Unclear Question Identification (UQI):} Given the user context ($c$), e.g., previous dialog turns, the current query ($q$), to classify whether it is proper to trigger the clarification question function for the current q.
\end{task}

A too frequent triggering would create extra huddle for the user to find the right information and may annoy her, while too little trigger would raise the risk of  misunderstanding user's search intents.
The rational of the task target, to ask for clarification or not, is quite complicated in real scenarios. It needs to take the consideration of user preference, search accuracy, and the experience the scenario would like to promote, in order to maximize the ultimate user satisfaction of the full conversational search system. In practice, at its rudimentary state, the unclear question identification task is often simplified as a standard classification task with human annotations on this intermediate task~\cite{aliannejadi2020convai3, trienes2019identifying}. 


\textbf{Clarification Question Selection/Generation} is to formulate the clarification question for the ambiguous user queries, e.g., when the dialog manager decided to use a clarification question in that turn, which best helps the user express and shape her information needs, with the ultimate goal of improving the overall search experience.

The clarification question can be obtained by \textit{ranking} a pre-given a set of candidate clarification questions, for example, either pre-given in an academic setting~\cite{rao2018learning} or mined and curated from search log with templates~\cite{zamani2020generating}. 

\begin{task}
Classification Question Selection:  Given the conversation context ($c$), the current query ($q$), and a candidate set of clarification questions $Q^\text{clari}$, to select to most proper clarification question $q^\text{clari} \in Q^\text{clari}$. 
\end{task}

On the other hand, it is often hard to obtain a candidate question set with high coverage. An alternative approach is to direct \textit{generate} $q^\text{clari}$ using natural language generation models~\cite{rao2019answer}. 

\begin{task}
Classification Question Generation:  Given the conversation context ($c$), the current query ($q$), to generate a clarification question $q^\text{clari}$.
\end{task}

This avoids the needs of a pre-constructed candidate question side, but also introduces the risk of low quality questions automatically generated, for example, from an natural language generation model. A practical way could be first automatically generate a large set of clarification questions and then filter down to high quality ones to construct the candidate question set for clarification question selection.

\subsection{Benchmarks}

As a new functionality in conversational IR, there is limited real user interaction data for clarification question tasks. There have been various efforts to create benchmarks for asking clarification questions using approximations from existing online data or human annotators. The benchmarks recently created can be categorized into three groups based on their origin: those from online QA forums,  from web search logs, and by crowd-sourcing.

\input{chapter_iir/forum_clariq}

\input{chapter_iir/forum_clariq_stat}

\textbf{Datasets Harvested from Online Forums.} One of the earliest approaches is to harvest the discussions on online forums and curate (context, clarification question) pairs~\cite{rao2018learning, rao2019answer}. These pairs include real user discussions that clarifying ambiguous user posts and provide a good starting point for reseaarch in asking clarification questions.

The \textit{StackExchange} dataset is constructed by Rao and Daum\'e III~\cite{rao2018learning} using the online discussions on StackExchange.com, an online question answering forum about topics like academic, Ubuntu, and latex, etc. There a user first posts a question about certain problems in these domains and, in the following discussions, other users often ask for more details in the post to help identify the technical details of the user's post. Rao and Daum\'e III use a set of hand-crafted rules to identify the clarification questions in the follow-up discussions and construct the (post, clarification question) pairs. In addition, they also identify the answer to the clarification question using the post editing history and direct responses. In total they obtained 77,097 (post, clarification question, answer) triples across three domains. 

The clarification question in the triple can be used as reference (``ground truth'') question for \textit{clarification question generation} task. In addition, Rao and Daum\'e III~\cite{rao2018learning} also formulate a ranking task. For 500 posts each from the develop (tune) and the test set, they constructed a candidate question set for each post using the clarification questions of its similar posts, retrieved by Lucene TF-IDF. They then recruited annotators to provide relevance labels for ten candidate questions randomly sampled from the candidate set. On average among these ten candidates, about 1-6 other questions labeled as valid clarification questions per post beside its own question.


Using a similar approach, Rao and Daum\'e III~\cite{rao2019answer} later curated the \textit{Amazon Home \& Kitchen} dataset using product description as the \textit{post}, questions asked to the product as the \textit{clarification questions}, and answers to the questions as the \textit{answer}. The (product description, clarification question, answer) triples are obtained from the Amazon question-answering dataset~\cite{mcauley2016addressing} and the Amazon reviews dataset~\cite{mcauley2015image}. 
% There is no candidate question set nor additional relevant labels associated with the Amazon dataset.

The examples of these two datasets are shown in Table~\ref{tab:forum_q}. Their statics are in Table~\ref{tab:forum_q_stat}. Both datasets can be used for clarification question selection and generation tasks. The candidate questions and extra relevance labels from the \textit{StackExchange} dataset might make it a more robust evaluation setting for question selection. All the posts in these two datasets are ambiguous or lacking some details by construction. They are not designed for the unclear question identification task.


\textbf{Datasets Created from Web Search Logs.} Zamani et al.~\cite{zamani2020mimics} released MIMICS, a benchmark created from the search logs in the clarification question function of Bing (Fig.~\ref{fig:clariQplane}). It includes the search query, the clarification question, and associated candidate answers displayed for the query, all from Bing's production systems. It includes three sub datasets, two with user interaction data (MIMICS-Click and MIMICS-ClickExplore) and one with human annotations (MIMICS-Manual).

For all three MIMICS datasets, the queries are harvested from Bing search log that 1) triggered the clarification question function, 2) passed their internal privacy and sensitivity filter. 
The clarification questions and answers are produced by certain variants of Bing production systems only using the information from the current query, i.e., no extra session context or user information is considered. The three MIMICS datasets differ in their questions, answers, and associated labels.

MIMICS-Click include clarification questions from an online production system that are displayed more than ten times during September 2019. The impression level, engagement level, and conditional click probability of its query-question pairs are normalized, post-processed, and released.

\input{chapter_iir/forum_mimics}

MIMICS-ClickExplore is similar to MIMICS-Click but reduces the potential system bias by including clarification questions from some exploration and online experiments in Septermber 2019.
The top clarification questions from their systems are presented to a certain set of Bing users in a A/B testing setup. All these questions that displayed more then ten times during that month is kept.

MIMICS-Manual is a smaller set of (query, clarification question) sampled similarly from the previous two but labeled with relevance levels by human annotators. The labels follow three Likert scale: 2 (Good), 1 (Fair), and 0 (Bad), with Good meaning the clarification question accurately address the clarification needs of the query.

The statistics of MIMICS datasets are listed in Table~\ref{tab:mimics}. Fig.~\ref{fig:clariQplane} shows an example from the Bing clarification question function.





\textbf{Datasets Curated by Crowd-Sourcing.} Another approach to construct clarification question benchmark is to employ crowd-source workers to curate clarification questions, answers, and labels for a given query.
Aliannejadi et al.~\cite{aliannejadi2019asking} developed Qulac  with crowd-sourced clarification questions and answers for the search queries and sub-topics (facets) from TREC Web Track 2009-2012. The ClariQ challenge~\cite{aliannejadi2020convai3} in ConvAI3 followed a similar approach with a slightly larger dataset.

Both Qulac and ClariQ, as inherited from TREC Web Track, include the relevance labels of documents for the original query. The document labels can be used to construct per query ambiguity labels based on the accuracy of initial retrieval, for example, a query with low-quality initial retrieval results is more likely to require clarification~\cite{ou2020clarifying}. 


    

\subsection{Modeling and Evaluation}

Recent research have developed various techniques for the unclear question identification and clarification question selection/generation tasks~\cite{aliannejadi2019asking, rao2018learning, rao2019answer, zamani2020generating}. In the rest of this section, for each task, we first describe a straightforward modeling solution with pretrained language models and the standard ways to evaluate them. As a rapid developing area, we only introduce the simplest modeling solution for these tasks and refer readers to check the literature for more up-to-date solutions. 

\textbf{Unclear Question Identification} can be formulated as a standard classification task. Given a query $q$ (or context/post based on the scenario)  and a candidate clarification question $q^\text{clari}$, one can leverage a pretrained model, e.g., BERT, to predict the probability of whether the $q$ needs clarification:
\begin{align}
    p(\text{needs clarify}|q) &= \text{MLP} (\text{BERT}(\text{[CLS]} q \circ \text{[SEP]} q^\text{clari} \text{[SEP]})),
\end{align}
with a MLP layer on top of the [CLS] representation from the BERT model.
The classifier can be fine-tuned using the per query ambiguity labels following standards in classification~\cite{ou2020clarifying}.
The \textit{evaluation} of the classifier can use its accuracy on this intermediate task, or its influence on the final user satisfaction when integrated in a conversational search system. 

\textbf{Clarification Question Selection} is often formulated as a ranking task, which is to rank the set of candidate questions $Q^\text{clari}$ based on their relevance to the given query. A straightforward solution is to use BERT to predict the ranking score for each pair:
\begin{align}
    f(q, q^\text{clari}) &=  \text{MLP} (\text{BERT}(\text{[CLS]} q \circ \text{[SEP]} q^\text{clari} \text{[SEP]})),
\end{align}
and rank the candidate questions based on this ranking score. The training of the ranking model can use standard ranking loss.
The \textit{evaluation} of the ranking model can follow the standard ranking evaluation with metrics such as Precision, MRR, and NDCG at different cut-off depth.

\textbf{Clarification Question Generation} can be done as simple as leveraging a pretrained NLG model that takes the input query and directly generate the clarification question. For example, one can use GPT-2~\cite{radford2019language} or other similar pretrained NLG model:
\begin{align}
    q^\text{clari} &= \text{GPT-2}(q),
\end{align}
where the model is fine-tuned using the oracle question as reference, and the generation results can be \textit{evaluated} using standard procedures in NLG. 



Ultimately, the effectiveness of the clarification question function is to be evaluate as part of the entire conversational search system.  It is costly to use an extra turn to clarify or the top space of the search result page to show the clarification panel.
The system needs to balance between the frequency of clarification questions and the risk of showing irrelevant responses, in order to achieve the best return of investment from adding the clarification question function. Evaluating the whole system end-to-end itself is a challenging and important research problem of it own, which is discussed in more detail in Chapter~\ref{chp:eval}.






==> chapter_iir/02_qreco.tex <==

\section{Leading CIR with Useful Suggestions}

The second type of system initiatives we discuss in this Chapter is to suggest useful questions that lead the conversation with the user \textit{within the same conversation topic}.
The suggestions can be potential next questions the user may ask in the next turn,  things the users may find interesting to continue her exploration, and queries that help user express her complicated information needs. 
All such suggestions can help carry the conversation with the user to the next stage in her information seeking or exploration journey of the current conversation topic, thus improve the user engagement and overall search experience.
The similar ``conversation recommendation'' function also plays a crucial role in chit-chat conversation systems in maintaining interesting dialogues with the user , e.g., it is a core function in the Sounding Board system, the winner of the first Alexa prize~\cite{fang2018sounding}, and has been adopted by various systems participated in later Alexa challenges, e.g., in Gunrock~\cite{yu2019gunrock}.

Many commercial search engines, including Google and Bing, have been presenting conversational leading suggestions since several years ago, as the ``People Also Ask'' feature. It helps promote more natural language questions and encourage more ``conversational-alike'' interactions with the search system, thus plays an important role in the shift from keyword search to more conversational experiences in commercial search engines. In this section, we use commercial web search as the example setup to discuss this conversation leading suggestion function. We start with describing this function and its typical solutions in Section~\ref{sec:paa_sys}. Then we discuss the needs of making the suggestions more useful in Section~\ref{sec:usefulness}, and recent explorations in training more conversation-leading suggestion system in Section~\ref{sec:convleading_model}.


\subsection{Question Suggestions in Commercial Search}
\label{sec:paa_sys}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{chapter_iir/gtr.pdf}
    \caption{An example of question suggestions for user query ``Nissan GTR price'' in the People Also Ask feature of a commercial search engine.}
    \label{fig:paa}
\end{figure}

Though commercial search engines are getting significantly better in empowering more natural language based search, many users still tend to issue single-turn keyword queries after years of experience with search engines inability to support multi-turn natural language questions. The People Also Ask (PAA) question recommendation feature is widely adopted in various commercial search engines to encourage users to experience the multi-turn natural language search capability.
An example of the PAA suggestion panel from Bing.com is illustrated in Figure~\ref{fig:paa}. Users can click on a question to reveal its answer and the PAA panel could expand with more question suggestions based on the clicked questions. It creates a mini conversational experience within the panel and advertises the search engine's capability in serving natural language questions to the user.

% Next we discuss how this PAA function can be implemented as a typical relevance-based ranking task, including its task setup and suggestion models.


% \textbf{Task Setup.} 
The question suggestion task can be formulated as a typical ranking problem: Give a user query $q$ and a set of candidate question suggestions $S=\{s_1,..s_i...,s_n\}$, to find the most proper suggestions. 


\textbf{Relevance Labels.} The target suggestions to display can follow the standard relevance notion in search: a good question suggestion is relevant to the user' search intent behind the query and could lead to a satisfied user click. Such  relevance labels can either be curated by human annotators, i.e. $y^\textbf{rel}=1$ if the annotators consider the suggestion $s$ is relevant to the query $q$, or harvested from user clicks in the search engine: $y^\text{click}=1$ if the user has clicked on $s$ for $q$.

\textbf{Suggestion Models} can be configured following the standard ranking system described in Chapter~\ref{sec:convsearch_bow}. For example, we can use a BERT-based ranking model~\cite{devlin2018bert} to rerank a BM25 retrieval candidate and pairwise learning to rank training~\cite{liu2009learning}:
\begin{align}
    f(q, s) &= \text{Linear} (\text{BERT}(\text{[CLS]}q \circ \text{[SEP]} s )), \\
    l &= \sum_{q} \sum_{(s^+, s^-) \in S^{q}} \text{max} (0, 1- (f(q, s^+) - f(q, s^-)).
\end{align}
The training pairs $(s^+, s^-) \in S^{q}$ are the relevant suggestion and irrelevant suggestion pairs of the corresponding query, based on either the relevance labels or click labels, or the mix of the two to form a multi-task setting.


\subsection{From Related to Useful Suggestions}
\label{sec:usefulness}


% the challenge of solely promoting relevance
    % 1) user preference shows not always
    % 2) duplicate with SERP's role, needs new information
    % 3) short term attention bait
Relevance is a natural offline quality metric for conversational question suggestions. It defines whether a suggestion is on topic and related to the query. An off-topic suggestion is unlikely to provide user a meaningful conversational search experience. However, as shown in recent research~\cite{rosset2020leading}, the offline relevance metric does not correlate well with online user preferences in question suggestion. A suggested question more relevant to the query is not always preferred by search engine users. An extreme example will be to suggest a question that is a paraphrase of the query, which is certainly on topic and relevant but does not provide user any new information.

In the first place, the goal of conversational question suggestion is not to satisfy user's information needs for the query of the current turn. That is the goal of the search results. If successful, user's information needs of the current turn should already be satisfied by the documents in the search result page; duplicating the same information in the question suggestions provide no additive gains.
Another concern of optimizing towards user click in question suggestions is risk of overfitting the system to short-term attention baits, things that attract user's eyeball but do not provide real value for the user. 

% the needs of new target and notation of usefulness: 
% usefulness goal and example
Recent research~\cite{rosset2020leading} in conversational question suggestion starts to go beyond relevance and introduces the notation of \textit{usefulness} to characterize whether a use will find value in the information the suggestions lead her into.  As the user's information needs of the current turn is to be satisfied by the retrieved documents or the system response, a useful suggestion should also capture things the user would be interested in \textit{the next step of her inquiry}.
As shown in Figure~\ref{fig:paa}, the targeted question suggestions for the query ``Nissan GTR price'' are those that help complete a task (``leasing deals''), weight options (``pros and cons about GTR''), further explore the topic (``ultimate streetcar''), or learn more details of the topic (``2020 GTR''). 
    
    


The first step to empower this conversation-leading experience is to develop new evaluation metrics that reflects this property beyond the traditional notion of relevance. 
The relevance can be considered as a prerequisite of a conversation-leading suggestion, but a relevant suggestion may not successfully lead the conversation. It may not provide forward-looking information, for example, the question suggestion ``what is GTR'' is a prequel information for the user query ``GTR Price''.   


\input{chapter_iir/tab_usefuleg}

\textbf{Usefulness Metric.} Rosset et at.~\cite{rosset2020leading} designed a new \textit{usefulness} metric to categorize the conversation-leading ability of question suggestions in Bing's People Also Ask function. They provide an annotation guideline for annotators to label a binary usefulness label of a (query, question suggestion) pair, while also including the categorizes of non-usefulness to help ensure annotation quality. The annotators then follow the guideline and assigned one of the following labels to each pair.
% metric
\begin{enumerate}
    \item \textbf{Misses Intent.} This category includes suggestions completely off-topic, poorly formatted, or not forming cohesive natural language questions. 
    \item \textbf{Too Specific.} This includes suggestions that only apply to a narrow portion of portion users, instead of the common public.
    \item \textbf{Prequel} suggestions are those about information a user properly already know when issuing the query thus do not provide new value to the user.
    \item \textbf{Duplicate with Query.} Suggestions that paraphrase the query are duplicates and do not provide useful new information.
    \item \textbf{Duplicate with Answer.} Suggestions whose information is already covered by the answer or other documents in the search result page do not provide new information to the user.
    \item \textbf{Useful} suggestions lead to valuable and new information for the user. There are multiple ways a suggestion to be useful. For example, it can help the user complete a task she has in mind, e.g., suggesting information about the next step in her task. It can also help the user re-frame her information needs or even shift her towards to right direction in finding the right answer. It can also be useful in helping the user to further explore the topic in the search process about things she may want to know more details.
    In general, a question is considered useful if it adds value about the search topic following a coherent line of thought, thus leads the conversation between the user and the search system.
\end{enumerate}


Examples of question suggestions in each category are listed in Table~\ref{tab:usefulness_eg}. Rosset et al.~\cite{rosset2020leading} demonstrated that in their online A/B test in Bing, the usefulness metric better correlates with online user preference. Users prefer suggestions from a system that shows higher usefulness metric offline, while not necessarily prefer systems whose suggestions are \textit{only}  relevant to the current query but not lead the conversation.




\subsection{Training Conversation-Leading Suggestion Systems }
\label{sec:convleading_model}


In the rest of this section, we describe the conversation-leading suggestion system developed for Bing People Also Ask in Rosset et al.~\cite{rosset2020leading}. Their main idea to improve the conversation-leading aspect, i.e., usefulness, of the system, is to train the suggestion model to suggest next turn questions in more conversation-alike user search sessions. We will first describe how they mine such conversation-alike sessions in the web search log and then how these training signals are injected to the suggestion model.



\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{chapter_iir/GenFilter.jpg}
    \caption{An example of the embedding based filtering in a five query session. A graph is created by connecting queries with an edge if their GenEncoder~\cite{zhang2019generic} embedding similarity is greater than 0.4, for example, between ``Flu Shot Codes 2018'' and ``How Much is Flu Shot?''. Queries that in the biggest connected component of the graph are kept. }
    \label{fig:gen_filter}
\end{figure}


\textbf{Mining Conversational-alike Sessions.} Web search logs include  a large amount of search sequences from users. Many of them capture user search trajectories when completing a task, learning a concept, or exploring a new topic. Learning from such search trajectories can help the system make more useful suggestions that help user proceed in the search process. On the other hand, search sessions are know to be very noisy. They are queries that co-appear in a certain time frame from a user, often by the 30 minute rule: breaking queries into different two sessions only if they are more than 30 minutes apart. However, within the 30 minute time frame,  the user may be multi-tasking or deviate from her initial task. Rosset et al.~\cite{rosset2020leading} developed an embedding based session mining technique that leverages a trained query embedding model, GEN Encoder~\cite{zhang2019generic}, to identify clean and topic coherent sessions that include high-quality search trajectories. 


\textit{Cleaning.} The first step of the session mining is to discard noisy queries. It starts from raw sessions grouped by the 30 minutes gap rule and discard navigational or mal-intent queries using standard query classification techniques. Then sessions with at least three queries and one satisfied user click are kept.

\textit{Coherent Filtering.} The second step is to filter the sessions only to the queries that form a coherent search trajectory. This is mainly conducted by leveraging the query embeddings the Bing's Gen Encoder~\cite{rosset2020leading}, which maps queries with similar search intent nearby in the embedding space. As illustrated in Figure~\ref{fig:gen_filter}, after obtaining the Gen Encodings of each query in a session, one can construct a graph by adding edges between query pairs deemed similar by their embedding, for example, if their cosine similarity is greater than 0.4, as studied in Zhang et al.~\cite{zhang2019generic}.  Then the largest connected sub-graph in the session is kept as the coherent part.  The rest queries are discarded as they are not on the same topic as the main component of the session. After this filtering, sessions with more than three queries are kept. 

This coherent filtering ensures the intents between queries in a session fall into the same conversation topic and thus reflect a meaningful search trajectory from the user.
In addition, Rosset et al.~\cite{rosset2020leading} further require one of the query in the cleaned coherent session has a successful interaction with the natural language answer from Bing QA system.
This favors sessions that include more natural language queries and are more information-seeking, rather than navigational or functional.


\input{chapter_iir/suggestion}


\textbf{Injecting Signals from Mined Sessions to Suggestion Models.} The mined conversation-alike sessions are used as training data for the suggestion system to learn the next-turn signal in their search trajectories. Rosset et al.~\cite{rosset2020leading} 
inject this next-turn information to the suggestion model using a learning task, \textit{Next Query Prediction}, where the model learns to predict user's next step in the search process.


\textit{Next Query Prediction} (NQP) task is that given a mined session $S=[q_1,...,q_{n-1},q_n]$, to predict the last query $q_n$ using all previous queries $q_{<n}$. For the BERT ranking model, it is to calculate a ranking score of $q_n$ for $q_{<n}$:
\begin{align}
    f^\text{NQP}(q_{<n}, q_n) &= \text{Linear}(\text{BERT}(\text{[CLS]} q_1 \text{[NQY]} \circ ... q_{n-1} \circ \text{[SEP]} \circ q_n )). 
\end{align}
In training, the actual next query $q_n$ is the positive target for $q_{<n}$.
To make sure the informativeness of the ranking task, the negatives are sampled from the queries that appears most frequently after $q_{n-1}$. The model is then trained using the standard learning to rank setup.


\textbf{Combing Relevance and Next Turn Prediction via Multi-Task.} The next query prediction task is combined with the relevance ranking task, described in Section~\ref{sec:paa_sys}, in a standard multi-task setting. These tasks are mixed equally in the training data and the BERT-based suggestion model learns both relevance and next-turn conversation-leading at the same time. In inference, the model outputs of the click prediction task is used to rank the candidate question suggestions~\cite{rosset2020leading}. All the other tasks are only used to inject the signals to the model for it to produce more useful suggestions.

Rosset et al.~\cite{rosset2020leading} show that the Next Query Prediction task with mined conversation-alike sessions is the source of more usefulness suggestions from the BERT-based model.
Adding the task significantly reduced the amount of Too Specific or Prequel suggestions, which is intuitive as those are unlikely to appear in user's search trajectory. The better offline usefulness also leads to more user engagement in their online A/B test with millions of Bing search users. Some examples of the suggestions from Bing's PAA production system before and after incorporating the conversation-leading and usefulness feature can be found in Table~\ref{tab:useful_suggestion_eg}.










==> chapter_iir/03_convreco.tex <==

\input{chapter_iir/tab_tiago}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{chapter_iir/TS_dialog_v1.pdf}
    \caption{An example dialog with topic shift in human conversations, from TIAGE~\cite{tiage}. The topic is shifted in the second to last turn, highlighted in \textcolor{ForestGreen}{\textit{green}}.}
    \label{fig:topic_shift_eg}
\end{figure}



\section{Switch Topics when Needed}

Another functionality to improve user's conversational search experience is to proactively shift conversation topics when needed. For example, when the conversation engagement is not ideal, the system can shift the discussion topic to some pre-given conversation goals~\cite{tang2019target}, such as  to ensure longer user engagement~\cite{tiage} and to recommend products~\cite{jannach2020survey}.
This is different from the conversation suggestion functionality discussed in last section as topic shift is to switch to a different conversation trajectory, while conversation suggestions are to help user advance the current trajectory.


% Various such real world scenarios demand the integration of goals in the conversation strategies and recent research has start to explore various ways to smoothly and effectively shift the conversation topics towards certain goals. 

Topic shift is a widely-adopted strategy in dialog systems. For example, XiaoIce, the chit-chat systems with millions of active users, employed a topic manager module that simulates the topic shift behaviors in human conversations~\citep{zhou2020design}. It first uses a classifier to detect whether to trigger the topic shift function, using features the indicates whether the Chit-chat outputs are failing or the user starts to lose interests. Once triggered, the topic shift function will retrieve a new topic from XiaoIce's database that may lead to better user engagements. The online experiments show that such topic shift function significantly improves user's engagement in XiaoIce.

% In conversational IR systems, the target of topic shift is slightly different from chit-chat systems, as the latter cares more about user engagement while CIR system's focus is to satisfy user's information needs and help users achieve their goals. 
In this section, we discuss recent explorations in making conversation systems more topic-aware and goal-oriented with the ability to proactively shift topics and thus guide the conversation. 
We mainly present two recent methods that approach this problem from three different ways: by implicitly modeling and mimic the topic shift in human conversations~\cite{tiage}, and by explicitly shifting topics through related keywords~\cite{tang2019target}.
These explorations are more in the chit-chat and goal-oriented setup, but their findings, datasets, and techniques could help boost the progress of topic shift studies in conversational IR systems. In addition, because of the infancy stage of this research area, we  focus more on describing their tasks and curated benchmarks rather than specific modeling solutions.


\subsection{Modeling Topic Shift in Human Conversations.}

 As shown in Figure~\ref{fig:topic_shift_eg}, human conversations naturally evolve to different topics through the discussion. A good and engaging discussion often includes several topics related at variant level and transits between them smoothly. 
 To enable conversation systems with the ability to shift between topics and improve user engagement, one intuitive approach is to learn from the topic shift behavior from human conversations.

% annotation shows there are rich topic shift behavior in persona conversation
Xie et al.~\cite{tiage} recruited annotators to manually annotate the topic shift behavior from the dev and test sets of the PersonaChat dataset~\cite{zhang2018personalizing}, which include dialogues between crowd-source workers chatting naturally with given personas.
The topic shift annotations are binary labels on each turn indicating whether there is a topic shift. 
The annotations show that topic shift is a quite common phenomena in human conversations. On average there are about one topic shift every 4-5 turns in the PersonaChat dataset. 

% provide that annotation labels as a benchmark, leads to two tasks
    % topic shift detection
    % topic shift aware response generation
\textbf{Benchmark.} The annotated datasets and the rest of PersonaChat form a benchmark to study topic-shift in dialog. The annotated part serves as supervised training/testing with explicit topic shift annotation. The rest can be used as weak supervision data as they contain dialogues from the same distribution but without topic shift annotation. The statistics of this dataset are listed in Table~\ref{tab:tiagostat}.  Though no explicitly conversation goals are assigned in PersonaChat nor TIAGE, one can use these datasets to explore dialog models' ability to naturally shift topics and continue meaningful conversations.
More specifically, Xie et al.~\cite{tiage} break down this into two sub-tasks: topic-shift detection and topic-shift response generation.


\textbf{Topic-Shift detection} is to predict whether it is proper to shift topic in the next turn, which is part of the dialog management component in a typical conversation system. 
Specifically, given the previous conversation turns, the task is to predict whether the next turn will have a topic shift in the annotated data.

The preliminary studies by Xie et al.~\cite{tiage} show that with the standard classification setup and pretrained model (T5~\cite{raffel2019exploring} in this case), it is not hard to classify the topic shift turns in retro-respective. The T5 classifier has access to previous turns and the next turn and is effective in determining whether they are for different topics. It reaches near 70\% F1 score when trained and evaluated using manual topic shift labels in the dataset.
To predict the topic shift in the future with only previous turns, on the other hand, is a much harder task. The same classifier's precision and F1 dropped more than half, to 0.34 Precision and 0.22 F1, if not using the information from the next turn.


\input{chapter_iir/tab_target_aware_stat}

\textbf{Topic-Shift response generation} is to generate a response that smoothly switches the topic.
It is formulated as an NLG task using the labeled topic shift turns in the human conversations as reference for training and evaluation. Xie et al.~\cite{tiage} measured the performance of several standard pretrained NLG models with and without fine-tuning and by using different portions of the TIAGE datasets. They found that it is not easy for recent NLG models to capture the subtle and noisy signals of topic shift in human conversations. Much new research is needed in this area.


\subsection{Explicit Topic Shifts Through Pre-defined Topics} 

Another way to formulate the topic shift task in conversation systems is to use keywords as explicit topics and using a pre-assigned topic as the conversation target. Tang et al.~\cite{tang2019target} formulate a such goal-oriented conversation scenario, where the system's goal is to shift the conversation with a user from an initial topic to a pre-given target topic. During the process, the system needs to balance the smoothness of the topic transition, as abrupt changes of topic yields awkward conversation experiences, and the effectiveness in achieving the conversation target, e.g., with fewer turns. 

\textbf{Benchmark.} 
Tang el al.~\cite{tang2019target} choose keywords as the explicit representations of conversation topics and construct a dataset also by deriving from the PersonaChat dataset~\cite{zhang2018personalizing}. They use a simple rule-based keyword extractor which uses TF-IDF and linguistic information to augment each turn with keywords. They also re-split the train/validation/test, allocating 500 conversations with more frequent keywords to the test set. The statistics of this dataset are shown in Table~\ref{tab:goal_conv_stat}. 
Tang el al.~\cite{tang2019target} then break down the whole system into two sub-tasks: \textit{Turn-Level Keyword Transition} and \textit{Keyword-Augmented Response Retrieval}.


\textbf{Turn-Level Keyword Transition.} This task focuses on predicting the keyword topics of the next turn given the conversation history. It breaks down the end-goal into turn level, which enables the usage of a wider range of conversational data that may not include a pre-given goals in the end turn. 
The primary focus of this turn level task is to ensure the smoothness between turns, e.g., by learning how human shift topics in natural conversations between turns.

Specifically, given the conversation utterances to the current turn $\{u_1,...,u_t\}$ and their annotated keywords $\{W^1,...,W^t\}$, with $W^i$ the set of keywords annotated to turn $u_i$, the task is to predict the keywords of the next turn $\{W^{t+1}\}$ from a given keyword vocabulary set $\mathbf{V}^w$, e.g., all keywords appeared in the training dataset.

The keyword prediction task can be conducted by learning a ranking function that scores the candidate keywords based on the context: $f(W^{t+1}; u_{<t}, W^{<t})$. Tang et al.~\cite{tang2019target} studies several approaches, including frequency based models, i.e., scoring the candidate keywords based on their correlation with keywords of the current turn in the training corpus, and neural based matching models~\citep{xiong2017knrm}. 

\textit{Injecting Target Goal in Keyword Transition.} In the turn level keyword prediction task, there is no information about the end goal nor guidance for the model to effectively shift towards the conversation goal. Tang et al.~\cite{tang2019target} inject the goal-awareness by simply restricting the candidate keyword set to only those that moving closer to the given target keywords, where the distance is measured by the ranking function. In the way one can restrict the candidate sets only to those can advance the conversation towards the final goal, among which the turn-level keyword prediction model selects the one with most smooth transition.




\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{chapter_iir/target_model.pdf}
    \caption{The illustration of the goal-oriented conversation system from Tang et al.~\cite{tang2019target}. The on-going conversation with a given target ``dance'' is shown in the left. The keyword selection module picks the most proper keyword in the space in each turn, to smoothly move the dialog trajectory to the target keyword, as illustrated in the right panel. The keyword-augmented response retrieval module selects the next response with the selected keyword (middle).}
    \label{fig:target_model}
\end{figure}


\textbf{Keyword-Augmented Response Retrieval.} The second task is to produce the response for the next turn, given the conversation history and the predicted keywords. It can be formulated as a retrieval problem that learns a neural ranking function $f(u_{t+1}; u_{<t}, W^{t+1})$ to retrieve responses from the corpus. 
It can also be formulated as a grounded natural language generation task where we use an NLG model to generate the response conditioned on previous turns and keyword topics. 




The two sub-modules can be combined together to empower the target-guided conversation scenario with smooth shifts between topic. As illustrated in Figure~\ref{fig:target_model}, ideally, a such system can select target topics  to discuss in the next turn that are relevant to previous conversation and also shift towards to the target topic. 
% That would form a smooth and target-guided trajectory in the keyword space and create a smooth topic shift with the keyword-augmented response retrieval system.



\textbf{Other Forms of Topic Representations.} Besides extract keywords, recent research has also explored the potential to use the knowledge graph entities and relations as explicit representation of conversation topics and topic shifts. In general a mentioning of a knowledge graph entity is considered as discussing that entity topic in the conversation turn. The shift between topics is modeled as a transition between entities through existing knowledge graph edges. The forms of knowledge graphs explored in recent literature include the standard RDF triples in knowledge graphs~\cite{wu2019proactive} and commonsense knowledge graph~\cite{speer2017conceptnet, zhang2019grounded, zhou2018commonsense}. 

Modeling topic shift using symbolic knowledge graphs shares similar benefits and challenges with many other symbolic systems. These systems are intuitive, explainable, and precise with benefits from high-quality knowledge graph. On the other hand, the coverage of such symbolic knowledge in real scenarios is often a problem. 
Research systems often either filter down to the conversations according to the coverage of chosen knowledge graphs~\cite{zhou2018commonsense} or employ crowd-source workers to construct dialogues following existing knowledge graph relations~\cite{wu2019proactive}. 
These restricts the variety of the result conversation topics, e.g., to a few specific domains where high quality knowledge graphs exist, for example, the movie domain~\cite{li2018towards, wu2019proactive}. 













==> chapter_iir/forum_clariq.tex <==
\begin{table}[]
    \centering
    \small
        \caption{Clarification questions harvested from online forums~\cite{rao2018learning, rao2019answer}} \label{tab:forum_q}
    \begin{tabular}{l|p{8cm}} 
    \hline
    \multicolumn{2}{l}{\textbf{From Stack Exchange}} \\ \hline
     Post Title    & Wifi keeps dropping on 5Ghz network \\ \hline
     Post Content   & Recently my wireless has been very iffy at my university. I notice that I am connected to a 5Ghz network, while I am usually connected to a 2.4Ghz everywhere else (where everything works just fine). Sometimes it reconnects, but often I have to run
`sudo service network-manager restart`. Is it possible a kernel update has caused this? \\ \hline
Clarification Question & what is the make of your wifi card? \\ \hline
Answer & Intel corporation wireless 7260 ( rev 73 ) \\ \hline
    \multicolumn{2}{l}{\textbf{From Amazon} \texttt{Home \& Kitchen}} \\ \hline
     Product Title    & T-fal Nonstick Cookware Set, 18 pieces, Red \\ \hline
     Product Content   & Easy non-stick 18pc set includes every piece for your everyday meals.
Exceptionally durable dishwasher safe cookware for easy clean up. Durable non-stick interior. Oven safe up to 350.F/177.C
 \\ \hline
Clarification Question & Are they induction compatible?
 \\ \hline
Answer & They are aluminum so the answer is NO. \\ \hline
    \end{tabular}

\end{table}

==> chapter_iir/forum_clariq_stat.tex <==
 \begin{table}[]
     \centering
     \small
          \caption{The statistics of (context, clarification question, answer) triples from StackExchange~\cite{rao2018learning} and Amazon Home \& Kitchen~\cite{rao2019answer} datasets.}
     \label{tab:forum_q_stat}
     \begin{tabular}{lllll}
     \hline
       & \textbf{Domain}   &  \textbf{Train} & \textbf{Tune/Dev} & \textbf{Test} \\ \hline
 \multirow{3}{*}{\textbf{StackExchange}} & \texttt{askubuntu} & 19,944 & 2493 & 2493 \\
 & \texttt{unix} & 10,882 &  1360 & 1360 \\
 & \texttt{superuser} & 30,852 & 3857 & 3856 \\ \hline
 \textbf{Amazon} & \texttt{Home \& Kitchen} & 19,119 & 2,435 & 2,305 \\ \hline
     \end{tabular}

 \end{table}

==> chapter_iir/forum_mimics.tex <==

\begin{table}[]
    \centering
        \caption{The statistics of MIMICS datasets, from Zamani et al.~\cite{zamani2020mimics}.}
    \label{tab:mimics}
    \begin{tabular}{llll}
    \hline
    & \texttt{Click} & \texttt{ClickExplore} & \texttt{Manual} \\ \hline
    
    \# unique queries & 414,362 & 64,007 & 2464 \\
\# query-clarification pairs  &414,362  &168,921 & 2832 \\
\# clarifications per query & 1 ± 0 & 2.64 ± 1.11  &1.15 ± 0.36 \\
% min \& max clarifications per query  & 1 \& 1  & 2 \& 89  & 1 \& 3 \\
\# candidate answers  & 2.81 ± 1.06  & 3.47 ± 1.20  & 3.06 ± 1.05 \\
% min \& max \# candidate answers  & 2 \& 5 2 \& 5  & 2 \& 5 \\
% \# query-clarification pairs with positive engagement  &71,188  &89,441  &N/A \\
% \# query-clarification pairs with low/medium/high impressions  &264,908 / 105,879 / 43,575 & 52,071 / 60,907 / 55,943 &  N/A \\ 
\hline
    \end{tabular}
\end{table}



==> tables/convsearch_notation.tex <==
\begin{table}
  %\caption{Table of Notation.}
  \label{tab:convsearch_notation}
  \begin{tabular}{ll}
  \hline
  \textbf{Symbol} & \textbf{Meaning} \\ \hline
  $\mathcal{T}$ & A conversational search topic that includes multiple turns of queries \\
  $q$ & A conversational query string \\
  $t$ & A term (word or sub word) \\
  $d$ & A document/passage \\
  $C$ & The corpus collection \\
  $\bs{q}$ &  The vector representation (discrete or continuous) of query $q$ \\
   $\bs{d}$ &  The vector (discrete or continuous) of document/passage $d$ \\
   $q^*$ & The manual oracle de-contextualized query rewrites \\
   $d^+, d^-$ & The labeled relevance and irrelevant documents \\
   $f(q, d)$ & The ranking/retrieval score for a query-document pair using function $f$ \\
  \hline
  \end{tabular}
\end{table}
